In-Context Learning with Transformers: Softmax Attention Adapts to Function Lipschitzness

A striking property of transformers is their ability to perform in-context learning (ICL), a machine learning framework in which the learner is presented with a novel context during inference implicitly through some data, and tasked with making a prediction in that context. As such, that learner must adapt to the context without additional training. We explore the role of softmax attention in an ICL setting where each context encodes a regression task. We show that an attention unit learns a window that it uses to implement a nearest-neighbors predictor adapted to the landscape of the pretraining tasks. Specifically, we show that this window widens with decreasing Lipschitzness and increasing label noise in the pretraining tasks. We also show that on low-rank, linear problems, the attention unit learns to project onto the appropriate subspace before inference. Further, we show that this adaptivity relies crucially on the softmax activation and thus cannot be replicated by the linear activation often studied in prior theoretical analyses.

==> NearestNeighbours/General.tex <==
\section{Pretraining Learns Scale of Attention Window}\label{sec:general}
One of our observations of the estimator used by attention, $h_{SA}$ (defined in Equation \ref{eq:attention}) is that it computes a nearest neighbours regression. We hypothesize that the role of pretraining is to select a neighbourhood within which to select tokens for use in the estimator. In this section we characterize this size. 
% We note that token embeddings are often normalized \cite{schlag2021linear}. 
First, we define function Lipschitzness and the families of function classes we study.
% It aligns with practice as token embeddings are often normalized \citep{}.
% The aforementioned assumptions are satisfied by a variety of function classes, specifically for our results we consider the following two function classes
% \begin{definition}[Lipschitzness of Function Class]
% The Lipschitzness of a function class $\mathcal{F}$ with domain $\mathcal{X}\subseteq \mathbb{R}^d$  is the largest Lipschitz constant of all functions in $\mathcal{F}$ over the domain $\mathcal{X}$, that is:
%     % Each $f_t\in \mathcal{F}$ is $L-$Lipschitz, that is 
%    \begin{align} \Lip(\mathcal{F}, \mathcal{X}) := \inf_{L \in \mathbb{R}} \{&L: f(x)-f( x')\le L\Vert x- x'\Vert \; \; \forall \; (x,x') \in \mathcal{X}^2, f\in \mathcal{F}\}.\nonumber
%     \end{align}
% \end{definition}
% Next, we define the function classes we consider in Theorem \ref{main:general}. 
% (maybe some remark about how the scaled identity result holds for larger class of functions. but this would come later)
\begin{definition}[Lipschitzness]\label{def:l}
    A function $f:\mathcal{X}\rightarrow\mathbb{R}$ has Lipschitzness $L$ if $L$ is the smallest number satisfying $ f(\bx)-f(\bx')\leq L\|\bx-\bx'\| $ for all $(\bx,\bx')\in\mathcal{X}^2$.
\end{definition}
\begin{definition}[Linear and 2-ReLU Function Classes]\label{def:f}
The function classes $\mathcal{F}^{\text{lin}}_{L}$ and $\mathcal{F}^{+}_{L}$ are respectively defined as:
    % Each $f_t\in \mathcal{F}$ is $L-$Lipschitz, that is 
\begin{align}
\mathcal{F}^{\text{lin}}_{L} &:= \{ f: f(\bx) = l\;  \mathbf{w}^\top \bx + b, \; \mathbf{w}\in \mathbb{S}^{d-1}, b, l \in [-L, L] \}, \nonumber \\ %\label{def:linearfn}\\
\mathcal{F}^{+}_{L} &:= \{ f: f(\bx) = l_1 (\mathbf{w}^\top \bx)_+ + l_2 (-\mathbf{w}^\top \bx)_+ + b, \; \mathbf{w}\in \mathbb{S}^{d-1}, (b,l_1,l_2) \in [-L, L]^2 \}. \nonumber %\label{def:relufn}
\end{align}
$D(\F^{\text{lin}}_{L}), D(\mathcal{F}^{+}_{L})$ are induced by drawing $\mathbf{w}\sim \mathcal{U}^d$ and $b, l, l_1, l_2 \stackrel{\text{i.i.d.}}{\sim} \text{Unif}([-L, L])$. 
%We also consider $D'(\mathcal{F}^{+}_{L})$, which is induced by $\mathbf{w}\sim \mathcal{N}(\mathbf{0}, \mathbf{I}_d)$ and $(l_1, l_2) \sim p$, where $p(l_1=l_2=L) = p(l_1=l_2=-L)=\nicefrac{1}{2}$.
 We say that these classes are \textbf{$L-$Lipschitz}, as the maximum Lipschitzness of any function in the class is $L$.
\end{definition}
% Note the assumed distribution over $\mathbf{w}$ is identical to that considered in \cite{ahn2023transformers} for only linear functions.
Here, $(z)_+ := \max(z,0)$.
Next, we assume the covariates are uniform on the
% make the following assumption regarding the distribution of the covariates that ensures that the softmax attention weights are a function of a weighted distance between $\bx_i$ and $\bx_{n+1}$
hypersphere\footnote{Our results in this section also extend to the case in which $D_{\bx} = \boldsymbol{\Sigma}\mathcal{U}^d$ for any $\boldsymbol{\Sigma}\succ \mathbf{0}_{d \times d}$; see Appendix \ref{app:full}.
% {\color{red}Most prior work assumes Gaussian distributions, and results along those lines (almost) show that inverting the covariance is a critical point for the optimization problem. Our distribution is a good approximation to the gaussian distribution in high dimensions, since most of the mass of a $\sigma^2$ variance gaussian lies at a radius of $\sqrt{\sigma d}$ anyway.}
}.
\begin{assumption}[Covariate Distribution]\label{assump:dists}
The covariate distribution $D_{\bx} = \mathcal{U}^d$.
\end{assumption}
% We note tokens are often normalized in practice \citep{kudo2018sentencepiece}.
Now we are ready to state our main theorem.
\begin{comment}
We begin with the following assumption that establishes symmetries in the function class. Then, we state our main results, followed by an informal proof sketch in a simplified setting.

\begin{assumption}\label{main:assumptions}
Every function $f$ in the function class $\F$ satisfies
    \begin{enumerate}
        \item $|f(x)-f(y)| \le L\Vert x-y\Vert ~\forall x, y, f$
        \item $\E_f \left[ f(x)f(y)\right] = \rho(x^\top y)~\forall x, y$ for some non-increasing $\rho$.
        \item For any isometry $\phi$ preserving the unit sphere, and $f\in \F$, we have $f\circ \phi\in \F$ and they both have the same probability. 
    \end{enumerate}
Also, the distribution $\X$ is uniform on the hyper-sphere.
\end{assumption}
% \textbf{Discussion of the Assumption:}
Assumption \ref{main:assumptions} requires that \textbf{(1)} the functions in $\F$ are $L-$Lipschitz, \textbf{(2)}  token labels become less correlated over the randomness in $f$ as the tokens move further apart, and \textbf{(3)} rotations and reflections are symmetries for the distribution $D(\F)$. These are general assumptions ...
These assumptions are fairly general - Lemmas (\ref{lem:linearsatisfiesassumption}) and (\ref{lem:nonlinearsatisfiesassumptions}) show that a natural distribution of linear and ReLU functions satisfy it. 

We next show that under this assumption, the attention a token pays to other tokens decays exponentially with the squared distance between the tokens.
\begin{lemma}\label{mainlem:assumptionssatisfyidentity}[Lemma \ref{lem:assumptionssatisfyidentity}]
    Under Assumption \ref{main:assumptions}, any minimizer of Equation \eqref{eq:loss} satisfies $\mathbf{M} = w_{KQ}I_d$ for some scalar $w_{KQ}$ and in particular, $$h_{SA}(\bx, {X}) = \sum_i\frac{f(\bx_i)e^{-w_{KQ}\Vert \bx-\bx_i\Vert^2}}{\sum_j e^{-w_{KQ}\Vert \bx-\bx_j\Vert^2}}$$ {\color{red} i think this eq should be in the proof sketch. also probably we should use $h_{SA}(\bx; w_{KQ} I_d)$

    TODO:  

i think we should just state the main theorem (or theorem(s) if separate for linear and relu) and not the lemmas and not the assumptions

so i think the section should look like this:

    1. define lipschitzness of function class `` We formalize the effect of function sharpness by  defining the Lipschitzness of the function class F as follows...''
    
    2. define linear and relu function classes.  define Dx and D-epsilon--maybe an assumption. i think we shouldn't use D(F), since all cases we use the uniform distribution over F (i've defined the distribution in the formulation section)

    3. state main theorem(s)

    3.5 interpret main thrm.

    4. proof sketch etc
    
    }
\end{lemma}
For linear functions, we can get tight upper and lower bounds for the optimal loss, given as
\begin{lemma}
    \label{main:linearbounds}[Lemmas (\ref{lem:linearbiasupperbound}), (\ref{lem:linearbiaslowerbound})]
    The loss $\uL(w_{KQ})$ is bounded as 
    \begin{equation}
        \frac{\underline{c_{\text{bias}}}L^2}{w_{KQ}^2}+ \frac{\underline{c_{\text{noise}}}\sigma^2 w_{KQ}^{\frac{d}{2}}}{n} \le \uL(w_{KQ})\le \frac{\overline{c_{\text{bias}}}L^2}{w_{KQ}^2} + \frac{\overline{c_{\text{noise}}} \sigma^2 w_{KQ}^\frac{d}{2}}{n}
    \end{equation}
    for constants $\underline{c_{\text{bias}}},\underline{c_{\text{noise}}},\overline{c_{\text{bias}}}$ and $\overline{c_{\text{noise}}}$ that .
\end{lemma}
This lemma allows us to characterize the solution $w_{KQ}$ as follows.
\end{comment}
\begin{theorem}%[Appendix \ref{app:full}]
\label{main:general}
Consider the pretraining loss \eqref{eq:loss} in the  cases wherein Assumption \ref{assump:dists} holds and tasks $f$ are drawn from \textbf{(Case 1)} $D(\mathcal{F}^{\text{lin}}_{L})$ or \textbf{(Case 2)} 
 $D(\mathcal{F}^{+}_{L})$. For $n=\Omega(1)$ and $\Omega(n^{-d/2}) \leq \sigma^2 \leq \mathcal{O}(nL^2)$, any minimizer $\mathbf{M}^*$ of \eqref{eq:loss} satisfies $ \mathbf{M}^* = w_{KQ} \mathbf{I}_d$
 \footnote{We further show in Appendix \ref{app:preliminaries} that $\mathbf{M}^*=w_{KQ}\mathbf{I}_d$, or $\mathbf{M}^*=w_{KQ}\boldsymbol{\Sigma}^{-1}$ when $D_{\bx}$ has covariance $\boldsymbol{\Sigma}$, holds for a broad family of rotationally-invariant function classes. 
    % not only $\mathcal{F}_{L}$ and $\mathcal{F}_{L_1,L_2}$. 
    }, where for $\Lambda\coloneqq \frac{nL^2}{\sigma^2}$, $\alpha\coloneqq \frac{1}{d+4}$ and $\beta \coloneqq \frac{1}{d+2}$:
    \begin{align}
      % \textbf{(1)}  & \; \Omega\Big(\Big(\frac{nL^2}{\sigma^2}\Big)^{\alpha}\Big) \le w_{KQ}\le \mathcal{O}\bigg(\Big(\frac{nL^2}{\sigma^2}\Big)^{2 \alpha \tfrac{d+2}{d}}\bigg),
      % % \hspace{0.1cm}\text{and}\hspace{0.1cm}  \uL(w_{KQ})\le \uO\left(\Big(\frac{\sigma^2L^d}{n}\Big)^{\frac{2}{d+2}}\right)
      % % \nonumber \\
      %  \textbf{(2)}  \;  \Omega\left(\Big(\frac{nL^2}{\sigma^2}\Big)^{\beta}\right) \le w_{KQ}\le \mathcal{O}\left(\Big(\frac{nL^2}{\sigma^2}\Big)^{2\beta}\right).
      %  % \hspace{0.1cm}\text{and}\hspace{0.1cm} \uL(w_{KQ})\le \uO\left(\Big(\frac{\sigma^2L^{d+2}}{n}\Big)^{\frac{2}{d+4}}\right).
      %  \nonumber
       \textbf{(Case 1)}  & \;\; \Omega\left(\Lambda^{\alpha}\right) \le w_{KQ}\le \mathcal{O}\left(\Lambda^{\frac{2\alpha}{1-\beta} }\right),\quad
      % \hspace{0.1cm}\text{and}\hspace{0.1cm}  \uL(w_{KQ})\le \uO\left(\Big(\frac{\sigma^2L^d}{n}\Big)^{\frac{2}{d+2}}\right)
      % \nonumber \\
       \textbf{(Case 2)}  \;\;  \Omega\left(\Lambda^{\beta}\right) \le |w_{KQ}|\le \mathcal{O}\left(\Lambda^{2\beta}\right).
       % \hspace{0.1cm}\text{and}\hspace{0.1cm} \uL(w_{KQ})\le \uO\left(\Big(\frac{\sigma^2L^{d+2}}{n}\Big)^{\frac{2}{d+4}}\right).
       \nonumber
    \end{align}
   %  where $w_{KQ}$ satisfies
   % \begin{equation} 
   % \end{equation}
\end{theorem}
Theorem \ref{main:general} shows that optimizing the pretraining population loss in Equation \ref{eq:loss} leads to attention key-query parameters that scale with the Lipschitzness of the function class, as well as the noise level and number of in-context samples. These bounds align with our observations from Figures \ref{fig:scaling} and \ref{fig:tradeoff}  that softmax attention selects an attention window that shrinks with the function class Lipschitzness, recalling that larger $w_{KQ}$ results in a smaller window. Further, the dependencies of the bounds on $\sigma^2$ and $n$ are also intuitive, since larger noise should encourage wider averaging to average out the noise, and larger $n$ should encourage a smaller window since more samples makes it more likely that there are samples very close to the query. To our knowledge, this is the {\em first result showing that softmax attention learns properties of the task distribution during pretraining that facilitate ICL}. Further, we have the following consequence for general inference tasks.

\begin{theorem}%[Appendix \ref{app:full}]
\label{thm:generalization}
    Suppose softmax attention is first pretrained on tasks drawn from $D(\F_L^+)$ and then tested on an arbitrary $L-$Lipschitz task, then the loss on the new task is upper bounded as $\uL \le \uO(\frac{L^2}{\Lambda^{\beta}}).$ Furthermore, if the new task is instead drawn from $D(\F_{L'}^+)$, the loss is lower bounded as $\uL\ge\Omega(\frac{L'^2}{\Lambda^{2\beta}})$ for $L' > L$ and $\uL\ge\Omega(\frac{\Lambda^{\beta d/2}}{n})$ for $L' < L$.
\end{theorem}
Theorem \ref{thm:generalization} shows that pretraining on $D(\F_L^+)$ yields a model that can perform ICL on downstream tasks {\em if and only if} they have similar Lipschitzness as $L$. Thus, learning Lipschitzness is both {\em sufficient and necessary} for ICL. If the Lipschitzness of the tasks seen during inference are much larger than those seen in pretraining, we will end up with biased estimates. On the other hand, if the Lipschitzness during inference is much lower, we are not optimally averaging the noise. Please see Appendix \ref{app:generalization} for the proof. 


% {\color{red} show corollary upper bounding generalization error of pretrained softmax attention on any new ICL task with Lipschitzness $\leq L$?}
% {\color{red} We note that the looseness of the bounds due to dimension-dependent factors is not important because...}

% The proof of Theorem \ref{main:general} involves a careful analysis of the presence of $\bx_i$'s in a neighborhood of radius $\frac{1}{\sqrt{w_{KQ}}}$  around $\bx_{n+1}$. We provide a simplified proof sketch next.

\subsection{Proof Sketch}\label{sec:proofoverview}
To highlight the key insights of our analysis, in this section we consider a modification of the softmax attention that exhibits important properties of the original. Note that this approximation is for illustration only; the above results use the original softmax attention -- see Appendices \ref{app:bias}, \ref{app:noise}, \ref{app:full}. For now, consider a function class $\F_L := \{ f: f(\bx) = L \mathbf{w}^\top \bx, \; \mathbf{w}\in \mathbb{S}^{d-1}\}$ of linear functions.
% Suppose further that $\boldsymbol{\Sigma} = \mathbf{I}_d$.

\para{(Temporary) modification of the softmax attention.}
Rather than averaging over every token with a weight that decays exponentially with distance, we consider a modification which \textit{uniformly} averages all tokens within a distance specified by $w_{KQ}=\Vert \mathbf{M}\Vert$. 
% Let $w_{KQ} = \Vert \mathbf{M}\Vert$, then 
From Lemma \ref{lem:assumptionssatisfyidentity}, without loss of generality (WLOG) we can consider $ \mathbf{M} = w_{KQ} \mathbf{I}_d$.
This means that, ignoring normalization, the weight assigned to $f(\bx_i)$ by the true soft-max attention is  $e^{-w_{KQ} \Vert \bx-\bx_i\Vert^2}$. That is, for all $\bx_i$ satisfying $\Vert \bx - \bx_i\Vert < \nicefrac{1}{\sqrt{w_{KQ}}}$, the assigned weights are all $\Theta(1)$, specifically in $(e^{-1},1]$.
% within a constant factor of each other. 
Meanwhile, for $\bx_i$ satisfying $\Vert \bx-\bx_i\Vert = \nicefrac{\sqrt{c}}{\sqrt{w_{KQ}}}$ for $c>1$, the weights are $e^{-c}$, decaying exponentially in $c$. This motivates us to consider a ``modified softmax attention" given by $h_{MSA}(\bx) := \sum_i \frac{f(\bx_i) \mathbbm{1}_i}{\sum_j \mathbbm{1}_j},$
where 
$\mathbbm{1}_j := \mathbbm{1}\{\Vert \bx-\bx_j\Vert < \nicefrac{1}{\sqrt{w_{KQ}}}\}$. In particular, $h_{MSA}(\bx)$  uniformly averages the labels of points within a Euclidean ball of radius $\nicefrac{1}{\sqrt{w_{KQ}}}$ around $\bx$, and ignores all others.

\para{The In-Context Loss.}
Since the (label) noise is independent of all other random variables, the pretraining loss from Equation \ref{eq:loss} can be decomposed into distinct weighted sums of labels and noise:
$$\uL(w_{KQ}\mathbf{I}_d) = \underbrace{\E_{f, \{\bx_i\}_i} \left( \sum_j \frac{(f(\bx_{n+1})- f(\bx_j))\mathbbm{1}_j}{\sum_j \mathbbm{1}_j}\right)^2}_{=:\uLb(w_{KQ})} + \underbrace{\E_{\{\bx_i\}_i, \{\epsilon_i\}_i}  \left(\sum_i \frac{\epsilon_i\mathbbm{1}_i}{\sum_j \mathbbm{1}_j}\right)^2}_{=:\uLn(w_{KQ})}.$$
We first upper and lower bound each of these terms separately, starting with $\uLb(w_{KQ})$.

\para{Noiseless Estimator Bias.} (Please see Appendix \ref{app:bias})
% Suppose the function class $\F$ is Lipschitz, satisfying 
% $$\forall ~ f, \bx, \bx', \hspace{0.2cm}|f(\bx)-f(\bx')|\le L\Vert \bx-\bx'\Vert.$$
% Then we have 
% We begin our analysis of $\uLb(w_{KQ}) $ by upper bounding it using the Lipschitzness of $\mathcal{F}$ (Assumption \ref{main:assumptions}) and the definition of $\mathbbm{1}_j$.
% \begin{align*} 
% \uLb(w_{KQ}) 
% % &= \E_{f, \{\bx_i\}} \left(f(\bx_{n+1}) - \frac{\sum_j f(\bx_j)\mathbbm{1}_j}{\sum_j \mathbbm{1}_j}\right)^2\\
% &\le \E_{f, \{\bx_i\}} \left(\frac{\sum_j L\Vert \bx_{n+1}-\bx_j\Vert \mathbbm{1}_j}{\sum_j \mathbbm{1}_j}\right)^2\le \E_{f, \{\bx_i\}} \left(\frac{\sum_j L\frac{1}{\sqrt{w_{KQ}}} \mathbbm{1}_j}{\sum_j \mathbbm{1}_j}\right)^2 = \frac{L^2}{w_{KQ}}\\
% \end{align*}
% Deriving a meaningful lower bound requires more work. Consider for instance a function class $\mathcal{F}$ consisting of constant functions, i.e. $f(x)=c$. Then $\uLb(w_{KQ}) =0$ for all distributions over $\mathcal{F}$ and all
% $w_{KQ}$. Thus, roughly speaking, to lower bound $\uLb(w_{KQ})$ away from zero we must leverage a lower bound on the complexity of the function class.
This term is the squared difference between an unweighted average of the token labels within a radius of $\bx$, and the true label. Take $w_{KQ} = \Omega(1)$. Then for large $d$, most of the points $\bx_i$ satisfying $\Vert \bx-\bx_i\Vert \le \nicefrac{1}{\sqrt{w_{KQ}}}$ lie on the boundary of the cap, that is, $\Vert \bx - \bx_i\Vert <\nicefrac{1}{\sqrt{w_{KQ}}}\implies \Vert \bx - \bx_i\Vert \approx\nicefrac{1}{\sqrt{w_{KQ}}}.$
This motivates us to approximate the set of points $\bx_i$ satisfying the above as coming from a uniform distribution over just the boundary of the cap. The center of mass of a ring of radius $\nicefrac{1}{\sqrt{w_{KQ}}}$ embedded on the surface of a hyper-sphere, is $\uO(\nicefrac{1}{w_{KQ}})$ from the boundary of a sphere, so the squared bias is $\Theta(\nicefrac{L^2}{w^2_{KQ}})$.
% Denote by $\uU_{\bx, \epsilon}$ the uniform distribution over $\bx'$ such that $\Vert \bx-\bx'\Vert = \epsilon$. Now we have
% \begin{align*} 
% \sum_i\frac{\mathbbm{1}_i f(\bx_i)}{\sum_j \mathbbm{1}_j} &= \sum_i\frac{\mathbbm{1}_i \mathbf{w}^\top \bx_i}{\sum_j \mathbbm{1}_j}\approx \mathbf{w}^\top \E_{\bx'\sim \uU_{\bx, \frac{1}{\sqrt{w_{KQ}}}}} \bx'=\mathbf{w}^\top \left(\E_{\bx'\sim \uU_{\bx, \frac{1}{\sqrt{w_{KQ}}}}} \left(\frac{\bx' + (2\bx\bx^\top -I)\bx'}{2}\right)\right)\\
% & =\mathbf{w}^\top\bx \left(\E_{\bx'\sim \uU_{\bx, \frac{1}{\sqrt{w_{KQ}}}}} \bx^\top\bx'\right)= \mathbf{w}^\top \bx \left(1-\frac{1}{w_{KQ}}\right)
% \end{align*}
% The squared difference is simply
% \begin{align*}
%     \E_{f, \{bx_i\}}\left[\left(f(\bx)-\sum_i\frac{\mathbbm{1}_i f(\bx_i)}{\sum_j \mathbbm{1}_j}\right)^2\right] 
%     &\approx \E_{f, \{bx\}} \left[\left(\mathbf{w}^\top \bx-\mathbf{w}^\top \bx \left(1-\frac{1}{w_{KQ}}\right)\right)^2\right]= \frac{L^2}{dw_{KQ}^2}\\
% \end{align*}


\para{Noise.} (Please see Appendix \ref{app:noise} for details) Since the noise is independent across tokens, expanding the square reveals that  $\mathcal{L}_{\text{noise}}(w_{KQ}) = \frac{\sigma^2}{\sum_j \mathbbm{1}_j}$, which is proportional to  the reciprocal of the number of tokens found within a $\nicefrac{1}{\sqrt{w_{KQ}}}$ radius of $\bx$. In Lemma \ref{lem:capbounds}, we derive bounds for the measure in this region and for now we ignore any finite-sample effects and replace the sum in the denominator with its expectation. This allows us to bound $\frac{1}{\sum_j \mathbbm{1}_j} = \Theta\big(\nicefrac{w_{KQ}^{\frac{d}{2}}}{n}\big)$ as long as $w_{KQ}\lesssim n^{2/d}$. 
% {\color{red} ... we also need something like $w_{KQ}\approx\Theta(1)$ for this to hold, right?}


\para{Combining the $\uLb$ and $\uLn$ terms.} (Please see Appendix \ref{app:full} for details)
Overall, we have $\uL = \uLb + \uLn$ with $\uLb= \Theta\big(\nicefrac{L^2}{w_{KQ}}\big)$ and $\uLn =\Theta\big( \nicefrac{w_{KQ}^{\frac{d}{2}}\sigma^2 }{n}\big)$. Minimizing this sum reveals that the optimal $w_{KQ}$ satisfies $w_{KQ} = \Theta\big((\nicefrac{nL^2}{\sigma^2})^{\frac{2}{d+2}}\big)$.  
% {\color{red}$\sigma$ here- also $\Lambda = \frac{nL^2}{\sigma^2}$ in the theorem? (not $\sigma$) }
% \begin{figure}[h]\label{fig:relative_weights}
%     \centering
%     \includegraphics[scale = 0.5, trim={3cm 0 3cm 0},clip]{Figures/bar.pdf}
%     \caption{\textbf{Left:} Plot of weights used in different estimators. In blue we see the weights of a linear regression estimator discussed in Remark \ref{rem:linearregression}. In gray and orange we see the weights from an attention layer with a small ``temperature" $1/\Vert \mathbf{M}\Vert = 10$ and large temperature $1/\Vert \mathbf{M}\Vert = 0.1$ respectively. \textbf{Center: }Rough upper and lower bounds for the bias term (shaded region), along with the noise variance (gray). \textbf{Right: }Overall upper and lower bound for the in-context loss. The horizontal dashed line establishes an upper bound for the optimal loss, while the vertical dashed lines establish lower and upper bounds for the parameter $w_{KQ}$ that can attain the optimal loss. TODO: label the axes}
%     \label{fig:enter-label}
% \end{figure}

% \begin{comment}
{
\subsection{Necessity of Softmax}
% {\color{red} should remove this because the lower bound on the loss is not worse that the upper bound on softmax loss.}
To further emphasize the importance of the softmax in Theorem \ref{main:general}, we next study the performance of an analogous model with the softmax removed. We consider {\em linear self-attention} \citep{von2023transformers,zhang2023trained,ahn2023transformers}, which  replaces the softmax activation with an identity operation. In particular, in the in-context regression setting we study, the prediction of $f(\bx_{n+1})$ by linear attention and the corresponding pretraining loss are given by:
% We denote this simplified version of self-attention  by $h_{LA}$, in particular:
\begin{align}\label{eq:linearattention}
h_{LA}(\bx_{n+1}) := \sum_{i=1}^n (f(\bx_i) +\epsilon_i){\bx_i^\top \mathbf{M}\bx_{n+1} }, \;\;
\mathcal{L}_{\text{LA}}(\mathbf{M}) := \E_{f, \{\bx_i\}_i, \{\epsilon_{i} \}_{i}} \left( h_{LA}(\bx_{n+1}) -f(\bx_{n+1})\right)^2. \nonumber
%\frac{\sum_j W_V\bx_je^{(\mathbf{W}_Q\bx_i)^\top (\mathbf{W}_K\bx_j)}}{\sum_j e^{(\mathbf{W}_Q \bx_i)^\top (\mathbf{W}_K \bx_j)}}
\end{align}
As discussed in Remark \ref{rem:scaling}, $h_{LA}(\bx_{n+1})$ cannot adapt an attention window to the problem setting. We show below that this leads it to  large ICL loss when tasks are drawn from $D(\mathcal{F}_L^+)$.
% We now have the following lower bound on the in-context loss of linear attention.
\begin{theorem}[Lower Bound for Linear Attention]\label{thm:negative-lin}
    % Consider any function class consisting of even functions, that is, any $\mathcal{F}$ such that for all $f \in \mathcal{F}$, $ f(\bx) = f(-\bx)$ for all $ \bx,\bx' \in \mathcal{X}$. Then $(\mathbf{W}_K, \mathbf{W}_Q)$ is a minimizer of $\mathcal{L}_{LA}(\mathbf{W}_K, \mathbf{W}_Q)$ if and only if $\mathbf{M} = 0$. 
    Consider pretraining on $\mathcal{L}_{\text{LA}}$ with tasks $f$ drawn from 
    $D(\mathcal{F}^{+}_{L})$ and covariates drawn from $\mathcal{U}^d$. Then for all $\mathbf{M}\in \mathbb{R}^{d\times d}$,  $\mathcal{L}_{LA}(\mathbf{M}) = \Omega({L^2})$.
\end{theorem}
% Theorem \ref{thm:negative-lin} shows that linear attention  cannot perform ICL on nonlinear function classes of the form studied in Theorem \ref{main:general}. 
This lower bound on  $\mathcal{L}_{LA}$ is strictly larger  than the upper bound on $\mathcal{L}$ from Theorem \ref{thm:generalization}, up to factors in $d$, as long as $\frac{\sigma^2}{n}\leq 1$, which holds in all reasonable cases. 
% This result formalizes our observation from theorem 
% The proof intuition comes from the fact that linear attention is particularly poorly suited for even functions, i.e. functions satisfying $f(\bx)\!=\!f(-\bx)\;\forall \bx$, since when $\bx$ is the query linear attention pays {\em negative} attention to $f(-\bx)$ even though this is the true label. 
% Although  $f\sim D(\mathcal{F}_{L}^+)$ is almost surely not even, we show that in expectation $f$ behaves as such. 
Please see Appendix \ref{app:lower} for the proof.
% On the other hand, as shown in Figure \ref{fig:scaling}, softmax attention  adapts its  attention window size to the function class, allowing ICL guarantees on a large class of functions with similar Lipschitzness.
% lower bound stems from the our 
% fact that the optimal $\mathbf{M}$ for linear attention when $\mathcal{F}$ consists only of even tasks, i.e. tasks satisfying $f(\bx)\!=\!f(-\bx)\;\forall \bx$, is $\mathbf{M}^*\!=\!\mathbf{0}_{d\times d}$. Please see Appendix \ref{app:lower} for details.
% that linear attention cannot learn anything meaningful when the tasks are odd functions which includes classes of the form $\mathcal{F}_{L_1,L_2}$ defined in Equation \ref{def:relufn} with $L_1=L_2$. 
% In contrast, we show in Lemma \ref{lem:} in Appendix \ref{} that the softmax estimator achieves 


}
% \end{comment}

\subsection{Experiments} Please see Appendix \ref{appendix:sims} for full details.

\para{Learning new tasks In-Context.} An important implication of our analysis is that for the function classes we consider, the attention estimator does not adapt to the function class beyond its Lipschitzness. In other words, an attention unit pretrained on linear tasks should have no issues generalizing for ICL to linear tasks (and vice versa), since for most points the nonlinearity will lie outside the attention window anyway. Figure \ref{fig:transfer_experiment} \textbf{(Left, Center)} demonstrate this transfer ability. We train two attention units, one with ReLU ($D(\F_L^+)$) pretraining tasks, and one with Linear ($D(\F_L)$) pretraining tasks. During pre-training we also compute the ICL error on $5$ test contexts at each iteration either drawn from $D(\F_L)$ or $D(\F_L^+)$. We run $10$ trials and aggregate our results over these trials. We set $d = 5, n = 200, \sigma = 0.03$ and draw $\{\bx_i\}_i$ independently and uniformly from the unit sphere. 
Observe that the test errors behave similarly for both function classes regardless of the pretraining function classes, since the pretraining classes have the same Lipschitzness.
% \textbf{(Left)} The ICL error on $D(\F_L)$ (Linear) tasks for an attention unit as it is pretrained on $D(\F_L)$ or $D(\F_L^+)$ (ReLU) tasks as a function of iteration. \textbf{(Right)} The ICL error on $D(\F_L^+)$ tasks as it is pretrained on $D(\F_L)$ and $D(\F_L^+)$. 

\para{Learning the scale of attention window.} We also demonstrate in Figure \ref{fig:transfer_experiment} \textbf{(Right)} that the attention window shrinks with increasing $n$ and $L$. Each point on the plot corresponds to an attention unit trained with tasks of a certain Lipschitzness using a varying number of tokens (depicted on the horizontal axis). The vertical axis depicts the norm $\Vert \mathbf{M}_K \mathbf{M}_Q\Vert$ after training. We optimize using the Adam optimizer with a learning rate of $10^{-3}$. The attention units are pretrained and tested on $D(\F_{L, \text{hills}})$.\footnote{Please see the Appendix \ref{appendix:sims} for a definition of $D(\F_{L, \text{hills}})$.} 
%Note that the attention window gets narrower with increasing $L$ and $n$ for the same noise level.

Plots to add:

4x1: relu, relu-nonisotropic, cos, cos non-isotropic

4x1: relu noise, cos noise, relu n, cos n

\begin{figure}
    \centering
    % \includegraphics[scale = 0.35, trim = {2cm 0 0cm 0}, clip]{Figures/transfer_linear_relu.pdf}
    \includegraphics[scale = 0.225]{Figures/transferrrr.pdf}
    \vspace{-3mm}
    \caption{\textbf{Left:} The ICL error on linear tasks of an attention unit as it is trained on ReLU and Linear functions as a function of training iteration number. \textbf{Center:} The ICL error on ReLU tasks of an attention unit as it is trained on ReLU and Linear functions as a function of training iteration number. \textbf{Right:} The reciprocal of the attention window as a function of the number of tokens for various choices of Lipschitzness.}
    \label{fig:transfer_experiment}
\end{figure}

\begin{comment}
{\color{gray}(old)


\noindent\textbf{Data.} 
We generate synthetic data by drawing tasks $f$ from  three function classes: (1) Generalized linear models (GLMs) with cosine link function with frequency $\omega$ ($\mathcal{F}_{\text{cos}}(\omega)$),
(2) two-layer ReLU teacher networks with ``scaling'' $\omega$ ($\mathcal{F}_{\text{ReLU},m}(\omega)$), and (3) linear models drawn from an $r$-dimensional subspace parameterized by $B_i\in \mathbb{O}^{d\times r}$ ($\mathcal{F}_{\text{lin}}(B_r)$). Formally,  $\mathcal{F}_{\text{cos}}(A,\omega) := \{f: f(x) = A\cos(\omega w^T x), w\in \mathbb{S}^{d-1}\}$,  $\mathcal{F}_{\text{ReLU}}:= \{f: f(x) = w_2^\top\text{ReLU}(W_1 x), W_1 \in \mathbb{S}^{(m\times d) -1},  w_2\in \mathbb{S}^{m-1}\}$, and  $\mathcal{F}_{\text{lin}}:= \{f: f(x) = w^T x, w = Bv, v\in \mathbb{S}^{r-1}\}$. 
For training, we draw tasks uniformly from each of these function classes -- for $\mathcal{F}_{\text{cos}}$, this amounts to drawing $\mathbf{w}\sim \mathcal{U}^{d-1}$, for $\mathcal{F}_{\text{ReLU}}$, this amounts to drawing $W_1 \sim \mathcal{U}^{m\times d}$ and $w_2\sim \mathcal{U}^{d}$, and  for $\mathcal{F}_{\text{lin}}$, this amounts to drawing $v\sim \mathcal{U}^{d}$.
% Denoting $p_{\text{sin}}$, $p_{\text{ReLU}}$ and ${\text{lin}}$ as the distributions over the functions in each of  We sample tasks from $\mathcal{F}_{\text{sin}}$ and $\mathcal{F}_{\text{lin}}$ by drawing a $w$ from $\mathcal{U}$, and sample from 
Unless otherwise noted, the features $x_i$ are drawn i.i.d. from $\mathcal{U}^{d}$, though we also include results for non-isotropic Gaussian $x_i$. 

% {\color{red} mayde also affine and/or constant functions}

\noindent\textbf{Training.} We train $\mathbf{W}_K, \mathbf{W}_Q,$ and $ W_V$ %and $W_P$
using Adam on the next-label prediction squared loss with a batch size of one context of length $n$ plus one query token per gradient update. 
We tune the learning rate for each architecture and for the median value of $L$ in each task setting (1,2,3), and hold it fixed for different values of $L$ for the same task setting and architecture to avoid the confounding effect of the learning rate on $\|\mathbf{M}\|$. We initialize $\mathbf{W}_K$ and $\mathbf{W}_Q$ using a Gaussian initialization with standard deviation $0.001$, and we train until convergence of the test error.  Please see Appendix \ref{appendix:sims} for more details. 

\noindent\textbf{Evaluation.} Every 500 training rounds, we evaluate the performance of the current model parameters on 500 fresh tasks with context length $n$ drawn from the same distribution used for training. The test error is the squared difference between the predicted label and the true query label averaged across all 500 contexts.
All reported statistics are averaged across 5 trails with different random seeds, with standard deviation provided.

\noindent\textbf{Results.} 
% \subsection{Results}
\textbf{Norm of $\mathbf{M}$ grows with  $L$.}
We start by discussing the results for the cosine  ($\mathcal{F}_{\text{cos}}(\omega)$) and two-layer ReLU ($\mathcal{F}_{\text{ReLU}}(\omega)$)  tasks. 
First we investigate the extent to which Theorem \ref{thm:Lipschitz} describes the behavior of the solution found in practice. Here, a simple calculation shows that the Lipschitz constants of $\mathcal{F}_{\text{cos}}(A, \omega)$ $\mathcal{F}_{\text{ReLU}}(\omega)$ are each equal to $\omega$, so we expect from Theorem \ref{thm:Lipschitz} that the norm of the $\mathbf{M}$ matrix resulting from training grows with $\omega$. 
Figures \ref{fig:grow_omega_cos} and \ref{fig:grow_omega_relu}  show that indeed this is the case for the cosine and ReLU tasks, respectively. These plots show that the $\omega$ used for training determines the relative norm of $\mathbf{M}$ after training for sufficiently long, with larger $\omega$ resulting in larger $\|\mathbf{M}\|_F$.

\textbf{Learning $L$ Improves Test Performance}
It remains to be seen whether learning L is actually useful.
To do this we compare with linear attention.
Figures \ref{fig:linear-comp-cos} and \ref{fig:linear-comp-relu} show that 

Linear attention is doing something fundamentally different than softmax attention.
We show in Appendix \ref{appendix:sims} that the norm of the key-query matrix in linear attention does not grow significantly during training with any value of $\omega$.
}


experiment ideas: 

% 1. for sin/cos functions: plot avg test error of $k$-nearest neighbors where $k$ varies along $x$ axis. softmax should be better than all these (will be straight horizontal line). can plot this for different frequencies, the best k should change with frequency. also plot test error of linear model.

% 2. norm of M varies with frequency of cos and L of MLP, not true for liner activation

3. plot showing some sort of behavior invariant to tasks that have the same L (train on linear, test on cos etc)

% Need to better specify the distribution over functions - what it means to get a random linear function (also in the appendix).
\end{comment}

==> NearestNeighbours/LowRank.tex <==
\section{Softmax Attention Learns Direction of Attention Window}\label{sec:LowRank}
% Much of the prior work in this area has focused on linear function classes, showing that such an attention layer can learn to do linear regression, and even that it can implement steps of gradient descent.
% \subsubsection{Gaussian X}
% TODO: Include basic analysis of Gaussian X with linear functions - show that the model adapts to different average Lipschitzness by considering the low rank $w$ case - here the function is 0-Lipschitz in some directions and this is reflected in $M$ being low rank.
Thus far, we have considered distributions over tasks that treat the value of the input data in all directions within the ambient space as equally relevant to its label. However, in practice the ambient dimension of the input data is often much larger than its information content -- the labels may change very little with  many features of the data, meaning that such features are spurious. 
This is generally true of embedded language tokens, whose embedding dimension is typically far larger than the minimum dimension required to store them (logarithmic in the vocabulary size) \citep{brown2020language}.
Thus, 
it is helpful to define a notion of ``direction-wise Lipschitzness'' of a function class to allow for analyzing classes that may depend on some directions within the ambient input data space more than others.
\begin{definition}[Direction-wise Lipschitzness of Function Class]
The Lipschitzness of a function class $\mathcal{F}$ with domain $\mathcal{X}\subseteq \mathbb{R}^d$ in the direction $\mathbf{w} \in \mathbb{S}^{d-1}$ is defined as
as the largest Lipschitz constant of all functions in $\mathcal{F}$ over the domain $\mathcal{X}$ projected onto $\mathbf{w}$, that is:
    % Each $f_t\in \mathcal{F}$ is $L-$Lipschitz, that is 
   \begin{align} \Lip_{\mathbf{w}}(\mathcal{F}, \mathcal{X}) := \inf_{L \in \mathbb{R}} \{&L: f(\mathbf{ww}^\top \bx)-f(\mathbf{ww}^\top \bx')\le L| \mathbf{w}^\top \bx- \mathbf{w}^\top \bx'| \; \; \forall \; (\bx,\bx') \in \mathcal{X}^2, f\in \mathcal{F}\}.\nonumber
    \end{align}
\end{definition}
% The Lipschitzness of $\mathcal{F}$ in the direction $\mathbf{w}$ can be thought of as the Lipschitzness of  $\mathcal{G}_{\mathbf{w}}:= \{g: g(z) = f(z\mathbf{w}), f\in \mathcal{F}, \; \forall z \in \mathbb{R}\}$.
\vspace{-0.2cm}
Using this definition, we analyze function classes consisting of linear functions 
% in e.g. \cite{ahn2023transformers,zhang2023trained,mahankali2023one}, 
with parameters lying in a subspace of $\mathbb{R}^d$, as follows:
% Next, we consider 
% function classes
% We show that softmax self-attention learns the directions in which the Lipschitzness of linear function classes is zero, allowing it to effectively reduce the in-context learning problem dimension. 
% % To do so, we consider the case in which the target function class consists of linear functions, as in the popular line of recent work \citep{}. 
% % However, unlike prior work, we (1) analyze softmax rather than linear self-attention, and (2) consider the general case in which 
% % We show that when 
% Specifically, we consider function classes of the form:
% \begin{align}
%     \mathcal{F}_{\mathbf{B}} \coloneqq \{ {f} : {f}(\bx) = \mathbf{a}^\top \mathbf{B}^\top \bx, \;\mathbf{a} \in \mathbb{S}^{k-1}, \; \forall \bx \in \mathbb{R}^d \}, \label{4}
% \end{align}
\begin{definition}[Low-rank Linear Function Class]\label{def:f-low-rank}
The function class $\mathcal{F}^{\text{lin}}_{\mathbf{B}}$ is defined as
    % Each $f_t\in \mathcal{F}$ is $L-$Lipschitz, that is 
% \begin{align}
% \mathcal{F}^{\text{lin}}_{ \mathbf{B}} &:= \{ {f}: {f}(\bx) = l \;\mathbf{a}^\top\mathbf{B}^\top \bx, \; \mathbf{w}\in \mathbb{S}^{d-1}, \; l \in [-L, L] \}, \nonumber \label{def:linearfn-}
% \end{align}
% \begin{align}
$\mathcal{F}^{\text{lin}}_{ \mathbf{B}} := \{ {f}: {f}(\bx) = \mathbf{a}^\top\mathbf{B}^\top \bx, \; \mathbf{a}\in \mathbb{R}^{d}\}$, %  \label{def:linearfn-}
% \end{align}
and $D(\F^{\text{lin}}_{\mathbf{B}})$ is induced by drawing $\mathbf{a}\sim \mathcal{N}(\mathbf{0}, \mathbf{I}_k)$.
\end{definition}
where $\mathbf{B}\in \mathbb{O}^{d\times k}$ is a column-wise orthonormal matrix. 
% Thus, $\mathcal{F}_{\mathbf{B}}$ consists of the set of linear regression tasks whose ground-truth regressors lie in the $k$-dimensional $\col(\mathbf{B})$. 
Since our motivation is settings with low-dimensional structure,
% in which the information content of inputs is far less than its input dimension, 
we can think of $k\ll d$.
% We assume that $D(\mathcal{F})$ is such that $\mathbb{E}[hh^\top ] = c_h I_k$ for some positive scalar $c_h$.
Let $\mathbf{B}_{\perp}\in \mathbb{O}^{d \times (d-k)}$ denote a matrix whose columns form an orthonormal basis for the subspace perpendicular to  $\col(\mathbf{B})$, and note that the Lipschitzness of $\mathcal{F}_{\mathbf{B}}^{\text{lin}}$ in the direction $\mathbf{w}$ is $L$ if $\mathbf{w}\in \col(\mathbf{B})$ and 0 if $\mathbf{w}\in\col(\mathbf{B}_{\perp})$. 
Observe that any function in $\F^{\text{lin}}_{\mathbf{B}}$ can be learned by projecting the input onto the non-zero Lipschitzness directions, i.e. $\col(\mathbf{B})$, then solving a $k\ll d$-dimensional regression.
% , so learning $\col(\mathbf{B})$ during pretraining would significantly  aid ICL on downstream tasks. 
% Thus, showing that softmax attention recovers $\col(\mathbf{B})$ during pretraining would help to explain how softmax attention can effectively in-context learn.
To formally study whether softmax attention recovers $\col(\mathbf{B})$, we assume the  covariates are generated as follows.
% We suppose the
\begin{assumption}[Covariate Distribution]\label{assump:low-rank}
 There are  fixed constants $c_{\mathbf{u}}\neq 0$ and $-\infty < c_{\mathbf{v}}  < \infty$ s.t. sampling $\bx_i \sim D_{\bx}$ is equivalent to
    $\bx_i = c_{\mathbf{u}} \mathbf{B} \mathbf{u}_i + c_{\mathbf{v}} \mathbf{B}_\perp \mathbf{v}_i$ where $ \mathbf{u}_i \sim \mathcal{U}^k$ and $ \mathbf{v}_i\sim \mathcal{U}^{d-k}$. 
    % \label{data-low-rank}.
% and $f_u \sim D(\mathcal{F}_{\mathbf{B}})$ is sampled by sampling  $u\sim \mathcal{U}^k$.
\end{assumption}
Assumption \ref{assump:low-rank} entails that the data is generated by latent variables $\mathbf{u}_i$ and $\mathbf{v}_i$ that determine label-relevant and spurious features. This may be interpreted as a continuous analogue of dictionary learning models studied in feature learning works \citep{wen2021toward,shi2022theoretical}.
% the projections of the data onto the the column spaces of $\mathbf{B}$ and $\mathbf{B}_{\perp}$ are each uniform on the respective unit hyperspheres. 
We require no finite upper bound  on $|c_{\mathbf{v}}|$ nor  $\frac{1}{|c_{\mathbf{u}}|}$, so the data may be dominated by spurious features.
% Still, the below result shows that softmax attention learns to zero-out the spurious features during pretraining.
% recovers the non-zero Lipschitzness  directions and zeros out the zero-Lipschitzness directions in the data.
% [parameterized by vectors] that lie in a fixed $k$-dimensional subspace of $\mathbb{R}^d$. Let $B\in \mathbb{R}^{d\times k}$ denote a matrix whose columns form an orthonormal basis for this subspace.

\begin{theorem}\label{thm:lin_low_rank}
Let $\mathbf{B}\in \mathbb{O}^{d\times k}$ and consider the pretraining population loss \eqref{eq:loss} with $f \sim D(\mathcal{F}^{\text{lin}}_{\mathbf{B}}) $. Suppose 
% tasks are drawn uniformly from $\mathcal{F}_{\mathbf{B}}$ and 
Assumption \ref{assump:low-rank} holds, as well as at least one of two cases: (Case 1) $\sigma=0$, or (Case 2) $n=2$.
% and let $\mathbf{B}_{\perp} \in \mathbb{O}^{d\times (d-k)}$ satisfy $B\mathbf{B}^\top + \mathbf{B}_{\perp} \mathbf{B}_{\perp}^\top = I_d$ for some $k \in [d]$. Suppose 
% That is, the columns of $\mathbf{B}_{\perp}$ form an orthonormal basis of the subspace perpendicular to the column space of $B$. 
    % Suppose the data  $\bx_i$ is generated as in \eqref{data-low-rank} for all $i\in [n+1]$. Let $w\in \mathbb{R}^d$ be a random vector satisfying $\mathbb{E}_{w}[ww^\top] = c_w B\mathbf{B}^\top$ for some $c_w>0$, and let $f_w(x) = w^\top x$. 
    % Suppose training is executed by sampling tasks from the induced distribution over $f_w$ with observed labels having noise variance $\sigma^2$. %and suppose the function class
    % let $M:=W_K^\top W_Q$.
    Then among all $\mathbf{M} \in \mathcal{M}:= \{\mathbf{M}\in \mathbb{R}^{d\times d}: \mathbf{M}=\mathbf{M}^\top, \|\mathbf{B}^\top \mathbf{M}\mathbf{B}\|_2 \leq \frac{1}{c_{\mathbf{u}}^2}\}$,
    the minimizer of the pretraining  population  loss \eqref{eq:loss}
    % \begin{align}
    %     \mathcal{L}(M) = \mathbb{E}_{f_u, \{\bx_i\}_{i\in [n+1]}, \{\epsilon_i\}_{i\in [n]} } \left[ \left(\frac{\sum_{i=1}^n  (f_u(\bx_i) - f_u(x_{n+1}) + \epsilon_i)e^{\bx_i^\top M x_{n+1}} }{\sum_{i=1}^n e^{\bx_i^\top M x_{n+1}} } \right)^2 \right]
    % \end{align}
    is $\mathbf{M}^* = c\mathbf{B}\mathbf{B}^\top$ for some $c \in (0,\frac{1}{c_{\mathbf{u}}^2}]$. 
\end{theorem}
% This 
Theorem \ref{thm:lin_low_rank} shows that softmax attention can achieve dimensionality reduction during ICL on any downstream task that has non-zero Lipschitzness only in $\col(\mathbf{B})$ by removing the zero-Lipschitzness features while pretraining on $\mathcal{F}_{\mathbf{B}}^{\text{lin}}$. To our knowledge, this is the {\em first result showing that softmax attention pretrained on ICL tasks recovers a shared low-dimensional structure among the tasks}. 
% To bridge this result with our results from Section \ref{sec:general}, we need to remove the condition  that either $\sigma=0$ or $n=2$; this is left as future work.
% Although $d$ may be smaller than $n$ in practice \citep{brown2020language}, it is still important to reduce the effective problem dimension for tasks whose sample complexity may scale superlinearly with $d$.
% In particular, 
% once we have $\mathbf{M} = c\mathbf{B}\mathbf{B}^\top$ for some $c>0$, pretraining reduces to finding the appropriate scale 
% reduces the dimension of the in-context linear regression task from $d$ to $k$. In particular, 
% Thus, in-context sample complexity depends only on $k$ rather than $d$.
% This phenomenon 
% shows clear evidence that softmax attention pretraining leads to learning properties of the label distribution,  rather than only the covariate distribution, and 
% can perhaps explain how transformers can effectively perform ICL in scenarios in which the number of in-context examples ($\approx \!10$)  is much smaller than the ambient data dimension ($\approx \! 1000$) \citep{brown2020language}.
% {\color{red} shows that again we learn info about labels during pretraining}
% , although further study is needed of transformers' ability to recover low-dimensional structure in data. Nevertheless,
% Indeed, we show empirically in Section \ref{sec:simulations} that one-layer softmax attention can again recover  the low-dimensional structure when the tasks are generalized linear models.

\para{Proof Sketch.} We briefly sketch the proof of Theorem \ref{thm:lin_low_rank}; please see Appendix \ref{app:low-rank} for the full version. Since $\mathbf{M}$ is symmetric, WLOG we write $\mathbf{M} = \mathbf{BP}\mathbf{B}^\top +  \mathbf{B}_{\perp}\mathbf{Q}\mathbf{B}_{\perp}^\top$ for symmetric matrices 
% $\mathbf{P}\in \mathbb{R}^{k\times k}$ and $\mathbf{Q} \in \mathbb{R}^{(d-k)\times (d-k)}$.
$\mathbf{P}$ and $\mathbf{Q}$.
Lemma \ref{lem:scalar-gen-low-rank} leverages the rotational symmetry of $\mathcal{F}_{\mathbf{B}}$ in $\col(\mathbf{B})$ to show that for any fixed $\mathbf{Q}$, the loss is minimized over $\mathbf{P}$ at a scaled identity, e.g. $\mathbf{P}=c\mathbf{I}_k.$
% if $\mathbf{P}\neq c\mathbf{I}_k$ for any $c>0$, then for any $\mathbf{Q}$ we have $\mathcal{L}(\mathbf{BP}\mathbf{B}^\top + \mathbf{B}_{\perp}\mathbf{Q}\mathbf{B}_{\perp}^\top)>\mathcal{L}(c\mathbf{B}\mathbf{B}^\top + \mathbf{B}_{\perp}\mathbf{Q}\mathbf{B}_{\perp}^\top) $ for some scalar $c \in (0,\frac{2}{c_{\mathbf{u}}^2}]$. 
% In other words, it is always better to not rotate the data in the ground-truth subspace 
% So WLOG we have $M = c\mathbf{B}\mathbf{B}^\top + \mathbf{B}_{\perp}Q\mathbf{B}_{\perp}^\top$. 
It remains to show that $\mathcal{L}(c\mathbf{B}\mathbf{B}^\top + \mathbf{B}_{\perp}\mathbf{Q}\mathbf{B}_{\perp}^\top)>\mathcal{L}(c\mathbf{B}\mathbf{B}^\top) $ whenever $\mathbf{Q}$ is nonzero. 
% To do so, 
% we exploit the fact that projections of $\bx_i$ onto $\col(\mathbf{B}_{\perp})$ {\em do not carry any information about the closeness of ${f}(\bx_i)$ and ${f}(\bx_{n+1})$}, i.e. the Lipschitzness of $f$ in directions in $\col(\mathbf{B})$ is zero. Thus, 
% we exploit the 
{Intuitively, if the attention estimator incorporates the closeness of $\mathbf{B}_{\perp}^\top \bx_{i}$ and $\mathbf{B}_{\perp}^\top \bx_{n+1}$ into its weighting scheme via nonzero $\mathbf{Q}$, this may improperly up- or down-weight ${f}(\bx_i)$}, since projections of $\bx_i$ onto $\col(\mathbf{B}_{\perp})$ {do not carry any information about the closeness of ${f}(\bx_i)$ and ${f}(\bx_{n+1})$}.
% if $ \bx_i^\top \mathbf{B}_{\perp} Q \mathbf{B}_{\perp}^\top \bx_{n+1} = \mathbf{v}_i^\top Q \mathbf{v}_{n+1} $ is large, and vice versa.

Using this intuition, we show that for any  fixed $\mathbf{Q}$ and $\{\mathbf{v}_i\}_i$ such that $\mathbf{v}_i^\top \mathbf{Q}\mathbf{v}_{n+1} \neq \mathbf{v}_{i'}^\top \mathbf{Q} \mathbf{v}_{n+1}$ for some $i,i'$, the attention estimator improperly up-weights $f(\bx_1)$, where $1 \in \arg\max_i  \mathbf{v}_i^\top \mathbf{Q} \mathbf{v}_{n+1}$ WLOG. In particular, 
the version of the pretraining population loss \eqref{eq:loss} with  expectation over ${\mathbf{a}}$, $ \{\mathbf{u}_i\}_i $ and $ \{\epsilon_i\}_i$ is reduced by reducing $\mathbf{v}_1^\top \mathbf{Q} \mathbf{v}_{n+1}$.
% as long as there is some $(i,i')$ such that $\mathbf{v}_i^\top Q \mathbf{v}_{n+1} \neq \mathbf{v}_{i'}^\top Q \mathbf{v}_{n+1}$. 
% In other words,  let $1 \in \arg\max_i  \mathbf{v}_i^\top \mathbf{Q} \mathbf{v}_{n+1}$ WLOG, then the estimator improperly upweights ${f}(\bx_{1})$ due to the closeness of $\bx_{1}$ and $\bx_{n+1}$ in $\col(\mathbf{B}_{\perp})$. 
The only way to ensure all $(\mathbf{v}_{i}^\top \mathbf{Q} \mathbf{v}_{n+1})_i$ are equal for all instances of $\{\mathbf{v}_i\}_i$ is to set $\mathbf{Q}=\mathbf{0}_{d \times d}$, so this $\mathbf{Q}$ must be optimal.

To show that reducing $\mathbf{v}_{1}^\top \mathbf{Q} \mathbf{v}_{n+1}$ reduces the loss with fixed $\{\mathbf{v}_i\}_i$, we define $\alpha_{i} \coloneqq e^{c_{\mathbf{v}} \mathbf{v}_{i}^\top \mathbf{Q} \mathbf{v}_{n+1}}$ for all $i\in [n]$ and show the loss' partial derivative with respect to $\alpha_{1}$ is positive, i.e.
\begin{align}
    \frac{\partial}{\partial \alpha_{1}}\left( \tilde{\mathcal{L}}(c, \{\alpha_i\}_i):= \mathbb{E}_{\mathbf{a}, \{\mathbf{u}_i\}_{i}, \{\epsilon_i\}_{i}} \left[ \bigg(\frac{\sum_{i=1}^n ({\mathbf{a}}^\top \mathbf{u}_i - {\mathbf{a}}^\top \mathbf{u}_{n+1} + \epsilon_i) e^{c c_\mathbf{u}^2 \mathbf{u}_i^\top \mathbf{u} } \alpha_i }{\sum_{i=1}^n  e^{c c_\mathbf{u}^2 \mathbf{u}_i^\top \mathbf{u}_{n+1} } \alpha_i } \bigg)^2  \right] \right) >0. \label{lsllll}
\end{align}
This requires a careful symmetry-based argument as the expectation over $\{\mathbf{u}_i\}_i$ cannot be evaluated in closed-form. To overcome this, we fix all $\mathbf{u}_i$ but $\mathbf{u}_{1}$ and one other $\mathbf{u}_{i'}\neq \mathbf{u}_{n+1}$ with $\alpha_{i'} < \alpha_1$. We show the expectation over $(\mathbf{u}_1,\mathbf{u}_{i'})$ can be written as an integral over $(\mathbf{y}_1,\mathbf{y}_2) \in \mathbb{S}^{k-1}\times \mathbb{S}^{k-1} $ of a sum of the derivatives at each of the four assignments of $(\mathbf{u}_1,\mathbf{u}_{i'})$ to $(\mathbf{y}_1,\mathbf{y}_2)$, and show that this sum is always positive. 
% This leverages the intuition that any ``bad'' assignment $\{\mathbf{u}_1=\mathbf{y}_1,\mathbf{u}_{i'}=\mathbf{y}_2\}$ for which increasing $\alpha_1$ could reduce the loss (e.g. if $\mathbf{y}_1=\mathbf{u}_{n+1}$) is outweighed by the other assignments, which cumulatively result in a larger increase of the loss due increasing $\alpha_1$.
Intuitively, any ``bad'' assignment for which increasing $\alpha_1$ reduces the loss is outweighed by the other assignments, which favor smaller $\alpha_1$. For example, if $\mathbf{y}_1=\mathbf{u}_{n+1}\neq \mathbf{y}_2$, and $\mathbf{u}_1=\mathbf{y}_1$ and $\mathbf{u}_{i'}=\mathbf{y}_2$, we see from \eqref{lsllll} that increasing  $\alpha_1$ can reduce the loss. However, the cumulative increase in the loss    on the other three assignments due to increasing $\alpha_1$ is always greater.
% $\{\mathbf{u}_{1}=\mathbf{y}_{1},\mathbf{u}_{i'}=\mathbf{y}_{2}\}, \{\mathbf{u}_{1}=\mathbf{y}_{2},\mathbf{u}_{i'}=\mathbf{y}_{1}\}, \{\mathbf{u}_{1}=\mathbf{y}_{1},\mathbf{u}_{i'}=\mathbf{y}_{1}\}, \{\mathbf{u}_{1}=\mathbf{y}_{2},\mathbf{u}_{i'}=\mathbf{y}_{2}\}$ occur with equal probability, we show that the sum of the derivatives conditioned on each of these events is positive, which implies the entire derivative is positive.
% Please see Appendix \ref{app:low-rank} for details.

% A single assignment of these tokens to points may have negative function value, meaning the pretraining loss could be improved by increasing the component of the weight matrix in the zero-Lipschitzness directions when considering only this particular assignment, but we show that the sum of all four function values is positive, for any two points

% So, these projections could cause the nearest neighbor estimate to improperly treat $\bx_i$ as a nearest  neighbor even though 


\begin{comment}
To do so, we decompose $M^\top \bx_i = cc_{\mathbf{u}} B\mathbf{u}_i + c_{\mathbf{v}} \mathbf{B}_{\perp}Q^\top \mathbf{v}_i$, which allows us to write 
\begin{align}
    e^{\bx_i^\top M \bx_{n+1}} = e^{ cc_{\mathbf{u}}^2 \mathbf{u}_i^\top \mathbf{u}_{n+1}  + c_{\mathbf{v}} \mathbf{v}_i^\top Q \mathbf{v}_{n+1} } = e^{ c' \mathbf{u}_i^\top \mathbf{u}_{n+1} } \alpha_i
\end{align}
where $\alpha_i \coloneqq c_{\mathbf{v}} \mathbf{v}_i^\top Q \mathbf{v}_{n+1}$ and $c':=cc_{\mathbf{u}}^2$. 
After  expanding the square in  the pretraining population loss \eqref{eq:loss} and taking expectation over ${f}$, and using the independence of the noise, we can use the above notation to re-write \eqref{eq:loss} as
\begin{align}
    \mathcal{L}(c\mathbf{B}\mathbf{B}^\top + \mathbf{B}_{\perp} Q \mathbf{B}_{\perp}^\top) 
    % &= \E_{f_u, \{\bx_i\}_i, \{\epsilon_{i} \}_{i}} \left(\frac{\sum_{ji1}^n (f_u(\bx_{n+1}) - f_u(\bx_i)- \epsilon_i) \; e^{\bx_i^\top M \bx_{n+1}}}{\sum_{i=1}^n e^{\bx_i^\top M \bx_{n+1}}}\right)^2 \nonumber \\
    & = \E_{ \{\alpha_i\}_i}\Bigg[ \underbrace{ \E_{ \{\mathbf{u}_i\}_i} \frac{\sum_{i,i'=1}^n (\mathbf{u}_i - \mathbf{u}_{n+1}) (\mathbf{u}_{i'} - \mathbf{u}_{n+1}) \; e^{c' (\mathbf{u}_i+\mathbf{u}_{i'})^\top \mathbf{u}_{n+1}} \alpha_i\alpha_{i'} }{\left(\sum_{i=1}^n e^{c' \mathbf{u}_i^\top  \mathbf{u}_{n+1}} \alpha_i \right)^2}}_{=:\tilde{\mathcal{L}}_{f}(c',\{\alpha_i\}_i)} \nonumber \\
    &\quad \quad \quad \quad \quad \quad + \underbrace{\sigma^2 \E_{ \{\mathbf{u}_i\}_i} \frac{\sum_{i=1}^n e^{2 c' \mathbf{u}_i^\top \mathbf{u}_{n+1}} \alpha_i^2 }{\left(\sum_{i=1}^n e^{c' \mathbf{u}_i^\top  \mathbf{u}_{n+1}} \alpha_i \right)^2}  }_{=:\tilde{\mathcal{L}}_{\epsilon}(c',\{\alpha_i\}_i)}\Bigg]. \label{qqq}
\end{align}
We proceed by showing that for any fixed $\{\alpha_i\}_i$ such that not all of the $\alpha_i$'s are equal, $\mathcal{L}_f(c',\{\alpha_i\}_i)+\mathcal{L}_\epsilon(c',\{\alpha_i\}_i) $ can be reduced by reducing the max $\alpha_i$. 
Moreover, if all $\alpha_i$'s are equal, the partial derivative of $\mathcal{L}_f(c',\{\alpha_i\}_i)+\mathcal{L}_\epsilon(c',\{\alpha_i\}_i) $ with respect to each $\alpha_i$ is zero. These two facts imply that $Q \in \arg\min \mathcal{L}_f(c',\{\alpha_i\}_i)+\mathcal{L}_\epsilon(c',\{\alpha_i\}_i) $ iff $Q$ is such that all $\alpha_i$'s are equal. The only way to achieve this for all instances of $\{\mathbf{v}_i\}_i$ is if $Q=0$, so the optimal $Q$ must be zero.

Suppose the $\alpha_i$'s are not all equal, and WLOG let $\alpha_1 =\max_{i\in [n]} \alpha_i$. We show that both $\frac{\partial \mathcal{L}_f(c',\{\alpha_i\}_i) }{\partial \alpha_1}$ and $ \frac{\partial \mathcal{L}_\epsilon(c',\{\alpha_i\}_i) }{\partial \alpha_1} $ are positive. Intuitively,

The cases $j=i$ and $j=1$, as well as showing $ \frac{\partial \mathcal{L}_\epsilon(c',\{\alpha_i\}_i) }{\partial \alpha_1} > 0 $,  require more involved computations but leverage the same basic symmetry principle. For example, showing that the noise derivative is positive entails showing that $\tilde{g}_{a,b}p_a p_b + \tilde{g}_{b,a}p_a p_b + \tilde{g}_{a,a} p_a^2 + \tilde{g}_{b,b} p_b^2 > 0$ for any $a,b\in [-1,1]^2$ and any probabilities $p_a,p_b$, where $\tilde{g}_{a,b}$ is the analogue of $g_{a,b}$ in \eqref{}. Please see Appendix \ref{app:low_rank} for the full proof. 
\end{comment}





% After some algebra, we obtain that
% \begin{align}
%     S_{i,j}\coloneqq \alpha_i \alpha_j \mathbb{E}_{ \{\mathbf{u}_{i'}\}_{i'\in [n]} } \left[ \frac{  (u_1 - \mathbf{u}_i)^\top  ( u_j -  u) e^{c_p (u_1^\top u + \mathbf{u}_i^\top u   +  u_j^\top u) }    }{(\sum_{i'=1}^n e^{c_p \mathbf{u}_{i'}^\top u }\alpha_{i'} )^3 }\right]
% \end{align}










% todo:make low dim gt regressor a, high dim ... w


% write $\mathcal{L}(c\mathbf{B}\mathbf{B}^\top + \mathbf{B}_{\perp}Q\mathbf{B}_{\perp}^\top)$ as:
% \begin{align}

% \end{align}
% The remainder of the proof relies on showing that if $c'\neq 0$ the loss of $M$ can always be improved by decreasing $|c'|$. In particular, we





% {\color{red} TODO: can this be extended to a simple nonlinear case? absolute value? possibly}


% \subsection{Negative Results}

% -Softmax prediction is not a gradient for linear functions. 

% -running one step of gd in the two-sided relu case would get you junk, maybe... or
% -softmax cannot implement the gradient in this case

% - how else to show something is not gd?


% show that trained transformers and 

% \begin{theorem}\label{thm:negative-grad}

    
% \end{theorem}








% \begin{comment}
%     extension to non-isotropic data:
    
% \end{comment}


% \vspace{-2mm}
\subsection{Experiments} 
% \vspace{-1mm}

Due to our results in Section \ref{sec:general} showing that softmax attention can learn an appropriate attention window scale when pretrained on nonlinear tasks, we hypothesize 
that it can also learn the appropriate directions during pretraining on nonlinear tasks.
% investigate whether softmax attention learns to ignore zero-Lipschitzness directions when trained on nonlinear function classes. 
To test this, we consider tasks drawn from low-rank versions of affine, quadratic and cosine function classes, in particular:
$\mathcal{F}^{\text{aff}}_{\mathbf{B}} := \{ {f}: {f}(\bx) = \mathbf{a}^\top \mathbf{B}^\top \bx + 2, \mathbf{a}\in \mathbb{S}^{k-1} \}$, $\mathcal{F}^{2}_{\mathbf{B}} := \{ {f}: {f}(\bx) = (\mathbf{a}^\top \mathbf{B}^\top \bx)^2, \mathbf{a}\in \mathbb{S}^{k-1} \}$ and  $\mathcal{F}^{\cos}_{\mathbf{B}} := \{{f}: {f}(\bx) = \cos(4\mathbf{a}^\top \mathbf{B}^\top \bx), \mathbf{a}\in \mathbb{S}^{k-1} \}$.
Each task distribution $D(\mathcal{F}^{\text{aff}}_{\mathbf{B}}),  D(\mathcal{F}^{2}_{\mathbf{B}} ), D(\mathcal{F}^{\cos}_{\mathbf{B}})$ is induced by drawing $\mathbf{a}\sim \mathcal{U}^k$.
We train $\mathbf{M}_K$ and $\mathbf{M}_Q$ with Adam with learning rate tuned separately for softmax and linear attention. We set $d=10$, $k=2$, $n=50$, and $\sigma=0.01$. 
% For both $\mathcal{F}^{\cos}_{\mathbf{B}}$ and $\mathcal{F}^{\text{affine}}_{\mathbf{B}}$  we 
% We sample 1 task per iteration by drawing
% $\mathbf{a}\sim \mathcal{U}^k$ and 
We draw
$\{\bx_i\}_{i=1}^{n+1}
% \stackrel{\text{i.i.d.}}{\sim} \mathcal{U}^{d\otimes (n+1)}
$ i.i.d. from a non-uniform distribution on $\mathbb{S}^{d-1}$ for each task, and draw one task per training iteration.
We draw $\mathbf{B}$ randomly at the start of each trial, and repeat each trial 5 times and plots means and standard deviations over the 5 trials.
We capture the extent to which the learned $\mathbf{M}=\mathbf{M}_K^\top\mathbf{M}_Q$ recovers $\col(\mathbf{B})$ via the metric $\rho(\mathbf{M},\mathbf{B}):= \frac{\|\mathbf{B}_\perp^\top \mathbf{MB}_\perp \|_2}{\sigma_{\min}(\mathbf{B}^\top \mathbf{M B})}$,  %\rho(\mathbf{M},\mathbf{B}):= 
where $\sigma_{\min}(\mathbf{A})$ is the minimum singular value of $\mathbf{A}$. % We refer to this as ``Representation Learning Error'' in the figures. 
For test error, we compute the average squared error on 500 random tasks drawn from the same distribution as the (pre)training tasks.
Please see Appendix \ref{appendix:sims} for more details.

\noindent\textbf{Results.} Figure \ref{fig:low-rank} shows that softmax attention recovers the low-rank structure when tasks are drawn from each of the three function classes, which leads to test error improving with the quality of the learned subspace. In contrast, linear attention does not learn any meaningful structure in these cases.


% Liam todo:
% experiments: make advait's labels larger, try to get his things to work for larger d and maybe sin, multiple trials at one seed, comp with linear for growth of M

% - experiments

% % --- cos and affine low rank (both work now)
% --- scale and test error for cos full rank. relu activation?

% - noise in appendix

% - fix lb proof

% - citations for formulation


% {\color{red}
% Liam todo:

% 1. experiments

% 2. clean appendix proof

% 3. deal with negative linear result

% 4. clean appendix RW

% minor: condense text, boldface, boldface matrices?

% }




% Although our theoretical results concern properties of minimizers of the population loss over contexts, there is no guarantee that practical training can find such minimizers 
% for two reasons: (i) the loss is nonconvex, so the gradient-based optimization methods  used in practice could converge to sub-optimal stationary points, and (ii) gradients of the loss cannot be computed exactly; practical methods must approximate them using a small number of contexts. 
% Despite these issues, we show in this section that our theoretical results well-describe the solutions found by practical training procedures under a number of data generative models.

% First, we show that 



% Maybe interesting hyperparameters:

% 1. data (normalized vs gaussian, isotropic vs not
% 2. noise
% 3. n

% Non-interesting hyperparameters:
% 1. batch size (always use 1)
% 2. optimizer (always use adam)
% 3. learning rate (tune)
% 4. d
% 5. r
% 6. initialization (always use gaussian, tune the scale)
% 7. number of training rounds
% 9. norm of normalized data: always use 1

% For all simulations we consider that the ground-truth labels are generated by generalized linear models of the form $f_t := \phi(w_t^T x)$, where $\phi:\mathbb{R}\rightarrow \mathbb{R}$ is a possibly non-linear activation function. We first consider the case in which $\phi:= \phi_{\omega,a}$ is the $\text{sin}$ function with frequency $\omega$ and amplitude $a$, i.e. $f_t(x) = A\text{sin}(\omega w^\top x)$. If $\|w_t\|_2 =1$ for all $w_t$, the Lipschitzness of this function class is exactly $A\omega$. We show that 
% % with particular activation functions. 

% \begin{figure}[h]\label{fig:grow_omega_cos}
% \centering
% \includegraphics[width=0.5\textwidth]{Figures/lowrank-cosine.pdf}
% \caption{
% % \textbf{Growth of $\|W_K^\top W_Q\|_F$ vs training iterations on cosine tasks with different values of $\omega$.}
% }
% \end{figure}

% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}[width=0.42\linewidth]{}
%         \centering
%         \includegraphics[height=1.41in]{Figures/lowrank-affine.pdf}
%         % \caption{Lorem ipsum}
%     \end{subfigure}%
%     \begin{subfigure}[width=0.4\linewidth]{}
%         \centering
%         \includegraphics[height=1.41in]{Figures/lowrank-quad.pdf}
%         % \caption{Lorem ipsum, lorem ipsum,Lorem ipsum, lorem ipsum,Lorem ipsum}
%     \end{subfigure}
%     \begin{subfigure}[width=0.9\linewidth]{}
%         \centering
%         \includegraphics[height=1.41in]{Figures/lowrank-cosine.pdf}
%         % \caption{Lorem ipsum, lorem ipsum,Lorem ipsum, lorem ipsum,Lorem ipsum}
%     \end{subfigure}
%     \vspace{-7mm}
%     \caption{Representation learning error $(\rho(\mathbf{M},\mathbf{B}))$ and test ICL error  during pretraining softmax and linear attention on tasks  from \textbf{Left:} $\mathcal{F}^{\text{affine}}_{\mathbf{B}}$, \textbf{Center:} $\mathcal{F}^{\text{2}}_{\mathbf{B}}$ , and \textbf{Right:} $\mathcal{F}^{\text{cos}}_{\mathbf{B}}$. } \label{fig:low-rank}
%     \vspace{-3mm}
% \end{figure*}
\begin{figure*}[t]
% \captionsetup[subfigure]{labelformat=empty}
%     % \centering
%     \begin{subfigure}{.333\textwidth}
%         \centering
%         \includegraphics[height=1.49in]{Figures/lowrank-affine.pdf}
%         % \caption{Lorem ipsum}
%     \end{subfigure}%
%     \begin{subfigure}{.333\textwidth}
%         \centering
%         \includegraphics[height=1.49in]{Figures/lowrank-quad.pdf}
%         % \caption{Lorem ipsum, lorem ipsum,Lorem ipsum, lorem ipsum,Lorem ipsum}
%     \end{subfigure}
%     \begin{subfigure}{.333\textwidth}
%         \centering
%         \includegraphics[height=1.49in]{Figures/lowrank-cosine.pdf}
%         % \caption{Lorem ipsum, lorem ipsum,Lorem ipsum, lorem ipsum,Lorem ipsum}
%     \end{subfigure}
\centering
\includegraphics[width=0.99\textwidth]{Figures/lowrank.pdf}
    \caption{Representation learning error $(\rho(\mathbf{M},\mathbf{B}))$ and test ICL error (mean squared error) during pretraining softmax and linear attention on tasks  from \textbf{Left:} $\mathcal{F}^{\text{affine}}_{\mathbf{B}}$, \textbf{Center:} $\mathcal{F}^{\text{2}}_{\mathbf{B}}$ , and \textbf{Right:} $\mathcal{F}^{\text{cos}}_{\mathbf{B}}$. } \label{fig:low-rank}
\end{figure*}

% \begin{figure}
%      \centering
%      \subfigure[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{graph1}
%          \caption{$y=x$}
%          \label{fig:y equals x}
%      \hfill
%      \subfigure[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{graph2}
%          \caption{$y=3\sin x$}
%          \label{fig:three sin x}
%      \hfill
%      \subfigure[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{graph3}
%          \caption{$y=5/x$}
%          \label{fig:five over x}
%         \caption{Three simple graphs}
%         \label{fig:three graphs}
% \end{figure}


% \begin{figure}[h]\label{fig:grow_omega_relu}
% \centering
% \includegraphics[width=0.5\textwidth]{omega_vs_iters_relu}
% \caption{\textbf{Growth of $\|W_K^\top W_Q\|_F$ vs training iterations on two-layer ReLU tasks with different values of $\omega$.}}
% \end{figure}

% \begin{figure}[h]\label{fig:attn_vs_omega_cos}
% \centering
% \includegraphics[width=0.5\textwidth]{attn_vs_omega_cos}
% \caption{\textbf{Example self-attention matrices $X_t^\top W_K^\top W_Q X_t$ after training on cosine tasks with different values of $\omega$.} As $\omega$ increases, the task labels become less flat, so the trained softmax self-attention does nearest neighbor regression with fewer neighbors, as shown by $X_t^\top W_K^\top W_Q X_t$ becoming more sparse.}
% \end{figure}

% \begin{figure}[h]\label{fig:test_error_cos}
% \centering
% \includegraphics[width=0.5\textwidth]{omega_vs_iters_cos}
% \caption{\textbf{Test error vs training iterations on cosine tasks for softmax attention (SA) and linear attention (LA) with different values of $\omega$.}}
% \end{figure}


% \textbf{Softmax attention can learn direction-wise Lipschitzness.}
% We say that a function class $\mathcal{F}$  has Lipschitzness $L_w$ on domain $\mathcal{X}$ in direction $w:\|w\|_2=1$ if $f(ww^\top x) - f(ww^\top x')\leq L_w\|x-x'\|_2$ for all $(x,x')\in \mathcal{X}^2$ and $f\in \mathcal{F}$.

% $\mathbf{B}\in \mathbb{R}^{d\times k}$ where $k< d$.





==> NearestNeighbours/Model.tex <==
\section{Preliminaries}  \label{sec:formulation}

% \para{Tasks and data.}
% This model was introduced by \cite{garg2022can} and has since been adopted by many other studies \citep{ahn2023transformers,zhang2023trained,von2023transformers,mahankali2023one,wu2018unsupervised,fu2023transformers,huang2023context,akyurek2022learning,cheng2023transformers,tian2023joma,bai2023transformers}.

% Works that study linear tasks: \citep{garg2022can,akyurek2022learning,zhang2023trained,wu2023many,von2023transformers,mahankali2023one,bai2023transformers,ahn2023transformers,fu2023transformers,raventos2023pretraining,huang2023context}.

\para{In-Context Learning (ICL).} Transformers have an astounding ability to adapt to novel contexts at inference time with no training. We study this phenomenon in the setting of regression. Specifically, in our model, each context consists of a set of feature vectors paired with scalar labels $\{\bx^{(t)}_i, f_t(\bx^{(t)}_i)\}$. The function $f_t$ used to label the features is drawn fresh for each context. During pretraining, the learner observes many such contexts to develop a pretrained model denoted by $\mathcal{A}(\{\{\bx^{(t)}_i, f_t(\bx^{(t)}_i)\}_i\}_t)$. At inference time, a new context $f$ is drawn - new features and new labels $\{\bx_i, f(\bx_i)\}$, as well as one special feature vector - the query $\bx$. The ICL objective is to use the task information implicit in the labelings of the other features to correctly label the query $\mathcal{A}(\{\{\bx^{(t)}_i, f_t(\bx^{(t)}_i)\}_i\}_t)(\bx, \{\bx_i, f(\bx_i)\})\to f(\bx)$.
%$\mathcal{A}\left(
%\begin{matrix}
%\{\bx^{(t)}_i, f_1(\bx^{(1)}_i)\}\\
%\{\bx^{(t)}_i, f_2(\bx^{(2)}_i)\}\\
%\vdots\\
%\{\bx^{(t)}_i, f_T(\bx^{(T)}_i)\}\\
%\end{matrix}
%\right)(\bx, \{\bx_i, f(\bx_i)\})\to f(\bx).$
We emphasize that $\mathcal{A}$ is pretrained using $f_1, f_2, \cdots, f_T$ and tested on $f$. This deviates from the traditional machine learning paradigm of training on data $\bx_1, \bx_2, \cdots, \bx_n$ to predict $f(\bx)$ for some fixed $f$. The difference
% , perhaps one of the key reasons for the success of the attention unit (ubiquitous in the transformer architecture), 
is that ICL happens {\em entirely in a forward pass}, so there is no training on $f$. Our inquiry focuses on the role of the softmax activation in the self-attention unit that enables such inference. First, we discuss the details of the self-attention architecture.

\para{The Softmax Self-Attention Unit.} 
We consider a single softmax self-attention head $H_{SA}(\cdot;\boldsymbol{\theta}) : 
\mathbb{R}^{(d+1)\times (n+1)}\rightarrow \mathbb{R}^{(d+1)\times (n+1)}$ 
parameterized by $\boldsymbol{\theta} \coloneqq \!(\mathbf{W}_K, \mathbf{W}_Q,\mathbf{W}_V)$, where  $\mathbf{W}_K, \mathbf{W}_Q,\mathbf{W}_V \in \mathbb{R}^{(d+1)\times (d+1)}$ are known as key, query, and value weight matrices, respectively.
% denoted by ${H}_{SA} : \mathbb{R}^{d \times (n+1)} \rightarrow \mathbb{R}^{d \times (n+1)}$. 
% This attention head receives a set of $n\!+\!1$ $d$-dimensional tokens, $\mathbf{Z} := [\mathbf{z}_1, \dots ,\mathbf{z}_{n+1}] \in \mathbb{R}^{d \times (n+1)}$, 
% that maps a set of tokens to another set of tokens.
Intuitively, for a sequence of tokens $\mathbf{Z}= [\bz_1,\dots,\bz_{n+1}]\in \bz^{(d+1)\times (n+1)}$,
the attention layer creates a ``hash map" where the key-value pairs come from key and value embeddings of the input tokens, $\{\bW_K \bz_i: \bW_V \bz_i\}$. Each token $\bz_i$ is interpreted as a query $\bW_Q\bz_i$, and during a pass through the attention layer, this query is matched with the keys $\{\bW_K\bz_j\}_j$ to return an average over the associated values $\{\bW_V\bz_j\}_j$ with a weight determined by the quality of the match (proportional to $e^{(\bW_K \bz_j)^\top (\bW_Q \bz_i)}$). Specifically,
{$H_{SA}( \mathbf{Z}; \boldsymbol{\theta}) = [h_{SA}( \mathbf{z}_1,\mathbf{Z}; \boldsymbol{\theta}), \cdots, h_{SA}( \mathbf{z}_{n+1},\mathbf{Z}; \boldsymbol{\theta})] $}, where
% maps a ``query'' token along with all other tokens to another vector in $\mathbb{R}^{d+1}$. To do so, $h_{SA}$ first computes key, query, and value embeddings of all tokens. For example, the key embedding of the $i$-th token is given by $\mathbf{W}_K \mathbf{z}_i \in \mathbb{R}^{d+1}$ and the query embedding of the $j$-th token is given by $\mathbf{W}_Q \mathbf{z}_j \in \mathbb{R}^{d+1}$.

% Next, for query token $\mathbf{z}_j$, the output of $h_{SA}(\mathbf{z}_j, \mathbf{Z}; \boldsymbol{\theta})$ is a convex combination of the value embeddings of all tokens, with the weight of the $i$-th value embedding determined by the alignment between the $i$-th key embedding and the $j$-th query embedding (which captures how much token $i$ ``attends to'' token $j$). These weights are exponentiated and normalized, such that the final output is:
\begin{equation}\tag{ATTN}\label{eq:attention}
h_{SA}(\mathbf{z}_i,\mathbf{Z}; \boldsymbol{\theta}) = \frac{\sum_{j=1}^n \left(\mathbf{W}_V \mathbf{z}_j \right)\; e^{(\mathbf{W}_K\mathbf{z}_j)^\top (\mathbf{W}_Q \mathbf{z}_i)}}{\sum_{i=1}^n e^{(\mathbf{W}_K \mathbf{z}_j)^\top (\mathbf{W}_Q \mathbf{z}_i)}} \in \mathbb{R}^{d+1}.
\end{equation}
With slight abuse of notation, we denote $h_{SA}(\mathbf{z}_j) = h_{SA}(\mathbf{z}_j,\mathbf{Z};\boldsymbol{\theta} )$ when it is not ambiguous. To study how this architecture enables ICL, we follow \cite{garg2022can} to formalize  ICL as a regression problem. Below we define the tokenization, pretraining objective and inference task.
% $\mathbf{Z}:=\{\mathbf{z}_i\}_i$ to another set of tokens $H_{SA}(\mathbf{Z}):= \{ h_{SA}(\mathbf{z}_i, \mathbf{Z}) \}_i$, such that each $h_{SA}(\mathbf{z}_i, \mathbf{Z})$ is a convex combination of value embeddings of all tokens $\{\mathbf{z}_i\}_i$ with weights determined by how much token $\mathbf{z}_j$ ``attends to'' token $\mathbf{z}_i$. In the setting with $\mathbf{Z}_t$ defined  
% and maps them another set of $n\!+\!1$ tokens via $ {H}_{SA}(\mathbf{Z}) = [h_{SA}(\mathbf{z}_1;\mathbf{Z}), \dots , {h}_{SA}(\mathbf{z}_{n+1},\mathbf{Z})]$ where each ${h}_{SA}(\mathbf{z}_{i};\mathbf{Z}) \in \mathbb{R}^d$. 
% In particular, the value embeddings are computed by linearly mapping each token via the weight matrix $\mathbf{W}_V$, and  the weights are computed by first linearly  mapping each token to key and query embeddings via weight matrices $\mathbf{W}_K$ and $\mathbf{W}_Q$, respectively. 
% The exponentiated alignment between the $j$-th key and $i$-th query gives a ``soft'' weight for the $j$-th value embedding for the $i$-th output token, that is then normalized by the sum of all weights for the $i$-th query. Formally:

\para{Tokenization for regression.} 
% \para{Using Attention to do Regression \textit{In-Context}} 
The learning model encounters token sequences of the form
\begin{align}
    \mathbf{Z} := \begin{bmatrix}
        \bx_{1} & \bx_{2} & \hdots & \bx_{n} & \bx_{n+1} \\
        f(\bx_{1}) + \epsilon_{1} & f(\bx_{2})+ \epsilon_{1}  & \hdots & f(\bx_{n}) + \epsilon_{n} & 0 \\
    \end{bmatrix} \in \mathbb{R}^{(d+1) \times (n+1)}, \label{z}
\end{align}
where the ground-truth labelling function $f$ maps from $\mathbb{R}^d $ to $ \mathbb{R}$ and belongs to some class $\mathcal{F}$, each $\epsilon_{i}$ is mean-zero noise, and the $i$-th input feature vector $\bx_i \in \mathbb{R}^d$ is jointly embedded in the same token with its noisy label $f(\bx_{i}) +\epsilon_{i} \in \mathbb{R}$. We denote this token $\mathbf{z}_{i}$. 
% Importantly, the ground-truth labelling function $f$ may vary across sequences.
% % Note that the $i$-th token embedding is $\mathbf{z}_{t,i}:= (\bx_{t,i}, f_t(\bx_{t,i}))$. 
% Note that the label of the $(n\!+\!1)$-th feature vector is masked as zero -- 
The ICL task is to accurately predict this label given the $n$ context tokens $\{ (\bx_{i}, f(\bx_{i}) + \epsilon_i) \}_{i=1}^n$, where $f$ may vary across sequences. The prediction for the label of the $(n\!+\!1)$-th feature vector is the $(d\!+\!1)$-th element of $h_{SA}(\mathbf{z}_{n+1})$ \citep{cheng2023transformers}, denoted 
$h_{SA}(\mathbf{z}_{n+1})_{d+1}$. Ultimately, the goal is to learn weight matrices such that $h_{SA}(\mathbf{z}_{n+1})_{d+1}$ is likely to approximate the $(n+1)$-th label on a random sequence $\mathbf{Z}$. 
% While prior work has focused on linear $f_t$, i.e. $f_t(\bx) = u_t^\top \bx$ for some $u_t\in \mathbb{R}^d$, with  $u_t$ having covariance equal to the identity \cite{} or the inverse covariance of $\bx_i$ \citep{ahn2023transformers}, we consider both  linear and nonlinear $f_t$ in Section \ref{sec:general} and linear $f_t$ with $u_t$ having possibly low rank covariance in Section \ref{sec:LowRank}.



\para{Pretraining protocol.} 
% For reasons we , we do not consider 
We study  what softmax attention learns when its weight matrices are {\em pretrained} using sequences of the form of \eqref{z}.
% , where the labelling functions belong to a particular function class $\mathcal{F}$.
% We consider function classes $\mathcal{F}$ 
These sequences are randomly generated as follows:
% functions uniformly from a function class $\mathcal{F}$ consisting of mappings $f_t : \mathbb{R}^d\rightarrow \mathbb{R}^d$. 
\begin{align}
   f \sim D(\mathcal{F}), \quad \bx_1,\dots,\bx_{n+1} \stackrel{\text{i.i.d.}}{\sim} D_{\bx}^{\otimes (n+1)}, \quad \epsilon_1,\dots,\epsilon_{n} \stackrel{\text{i.i.d.}}{\sim} D_\epsilon^{\otimes (n+1) }
\end{align}
where $D(\mathcal{F})$ is a distribution over functions in $\mathcal{F}$, $D_{\bx}$ is a distribution over $\mathbb{R}^d$, and $D_\epsilon$ is a distribution over $\mathbb{R}$ with mean zero and variance $\sigma^2$. The token embedding sequence $\mathbf{Z}$ is then constructed as in \eqref{z}. 
Given this generative model, the pretraining loss of the parameters $\boldsymbol{\theta} = (\mathbf{W}_Q, \mathbf{W}_K, \mathbf{W}_V)$ is the expected squared difference between the prediction of softmax attention and the ground-truth label of the $(n\!+\!1)$-th input feature vector in each sequence, namely
\begin{equation}
% \tag{ICL}
\label{eq:loss0}
\bar{\uL}(\boldsymbol{\theta}) := \E_{f, \{\bx_i\}_i, \{\epsilon_{i} \}_{i}} \left(h_{SA}(\mathbf{z}_{n+1})_{d+1}-f(\bx_{n+1})\right)^2.
\end{equation}
% \para{Reparameterization.} 
% Following \cite{cheng2023transformers}, and others, 
We next reparameterize the attention weights to make \eqref{eq:loss0} more interpretable. 
First, note that this loss is not a function of the first $n$ columns of $\mathbf{W}_V$, so without loss of generality, we set them to zero. For the last column, we show in Appendix \ref{app:preliminaries} that any minimizer of \eqref{eq:loss0} in the settings we consider must have the first $d$ elements of this last column equal to zero. As in \cite{cheng2023transformers}, we fix the $(d\!+\!1,d\!+\!1)$-th element of $\mathbf{W}_V$, here as 1 for simplicity. In the same vein, we follow \cite{ahn2023transformers,cheng2023transformers} by setting the $(d\!+\!1)$-th row and column of $\mathbf{W}_K$ and $\mathbf{W}_Q$ equal to zero. To summarize, the reparameterized weights are:
\begin{align}
    \mathbf{W}_V = \begin{bmatrix}
        \mathbf{0}_{d \times d} & \mathbf{0}_{d\times 1} \\
        \mathbf{0}_{1\times d} & 1 \\
    \end{bmatrix}, \quad  \mathbf{W}_K = \begin{bmatrix}
        \mathbf{M}_K & \mathbf{0}_{d\times 1} \\
        \mathbf{0}_{1\times d} & 0 \\
    \end{bmatrix}, \quad  \mathbf{W}_Q = \begin{bmatrix}
        \mathbf{M}_Q & \mathbf{0}_{d\times 1} \\
        \mathbf{0}_{1\times d} & 0 \\
    \end{bmatrix}
\end{align}
where $\mathbf{M}_K, \mathbf{M}_Q \in \mathbb{R}^{d\times d}$.
Now, since our goal is to reveal properties of minimizers of the pretraining loss, rather than study the dynamics of optimizing the loss, without loss of generality we can define $\mathbf{M} := \mathbf{M}_K^\top \mathbf{M}_Q$ and re-define the pretraining loss \eqref{eq:loss0} as a function of $\mathbf{M}$. Doing so yields:
% With this choice of $\mathbf{W}_V$, we can re-write the pretraining population loss as follows:
    \begin{equation}
\tag{ICL}
\label{eq:loss}
\uL(\mathbf{M}) := \E_{f, \{\bx_i\}_i, \{\epsilon_{i} \}_{i}} \left(\frac{\sum_{i=1}^n (f(\bx_i)+ \epsilon_i) \; e^{\bx_i^\top \mathbf{M} \bx_{n+1}}}{\sum_{i=1}^n e^{\bx_i^\top \mathbf{M} \bx_{n+1}}}-f(\bx_{n+1})\right)^2.
\end{equation}
\noindent\para{Interpretation of the pretraining loss.}\vspace{-2.6mm} The loss \eqref{eq:loss} clarifies how softmax attention can be interpreted as a {nearest neighbors regressor}.
Under the assumption that $\bx_i^\top \mathbf{M} \bx_{n+1}$ is a proxy for the distance between $\bx_i$ and $\bx_{n+1}$ (which we formally show in Section \ref{sec:general}), the softmax attention prediction is a convex combination of the noisy labels with weights determined by the closeness of $\bx_i$ to $\bx_{n+1}$, such that the labels of points closer to $\bx_{n+1}$ have larger weight. 
% As we see in Figure \ref{fig:scaling}. 
Moreover, the decay in weights on points further from $\bx_{n+1}$ is exponential and controlled by $\mathbf{M}$, which effectively defines a neighborhood, or attention window, of points around $\bx_{n+1}$ whose labels have non-trivial weight.
% , allowing $\mathbf{M}$ to 
% , it i, based on how quickly the labels are changing.
% to prioritize only the closest points when $f$ changes sharply and the noise level is small, and to average over a larger neighborhood in the opposite case. 
As we have observed in Figure \ref{fig:scaling},
our key insight is that pretrained $\mathbf{M}$ \textbf{scales this attention window with the Lipschitzness of the function class.}
Generally speaking, larger $\mathbf{M}$ entails averaging over a smaller window and incurring less bias due to the function values of distant tokens in the estimate, while smaller $\mathbf{M}$ entails averaging over a larger window, resulting in larger bias due to distant token labels, but a smaller noise variance.  Figure \ref{fig:tradeoff} further depicts this tradeoff.
% In the following sections we formally show that $\mathbf{M}$ learns to appropriately calibrate the neighborhood size under particular choices of $\mathcal{F}$ and $D_{\bx}$.

\begin{remark}[Extreme cases and the softmax advantage]\label{rem:scaling}
    Consider the following two settings.

    \noindent\textbf{Constant functions.} If each of the functions the attention unit sees in pretraining is constant, as in the \textbf{Left} column of Figure \ref{fig:scaling}, it is best to consider a huge attention window, that is, take $\mathbf{M} = \mathbf{0}_{d\times d}$ as this results in a uniform average over all the noisy token labels. %The resulting estimator is unbiased, and it has the best possible variance of $\sigma^2/n$.

    \noindent\textbf{Rapidly changing functions.} If the pretraining functions change rapidly, as in the \textbf{Right} column of Figure \ref{fig:scaling}, attending to a distant token might serve only to corrupt the estimate at the target. Consider another example in which the input tokens are used to construct Voronoi cells on the surface of the hypersphere and the label for a new token in a cell is the label of the token used to construct that cell. The optimal estimator would attend only to the single nearest token since this incurs error only from label noise.

    % We illustrate examples in Figure \ref{fig:scaling}, where as we go from left to right the function Lipschitzness increases. This results in the need for a smaller attention window \textbf{(Middle Row)}.
%% \end{remark}

%% gin{remark}[The softmax advantage]\label{rem:linearregression}
    \noindent\textbf{Advantage of the softmax.} To further highlight the property of softmax that enables the behaviour discussed above, we compare with linear attention \citep{von2023transformers,zhang2023trained,ahn2023transformers}, whose estimator can be written as $h_{LA}(\bx) = \sum_i (f(\bx_i) +\epsilon_i) \bx_i^\top \mathbf{M}  \bx$, up to a universal scaling due to the value embedding.
    % the least squares estimator. The least squares estimator can also be written as $\hat f(\bx) = \sum_i \bx \left(\sum_j \bx_j \bx_j^\top \right)^{-1}  \bx_i f(\bx_i)$, which is a weighted combination of the function values at neighbouring points $\bx_i$, with weights determined by $\bx \left(\sum_j \bx_j \bx_j^\top \right)^{-1}  \bx_i$. 
    This is again a weighted combination of labels, but one that does not allow for adapting an attention window -- any scaling of $\mathbf{M}$ does not change the relative weights placed on each label -- unlike softmax attention. Please see Figure \ref{fig:scaling} \textbf{(Middle Row)} for a comparison of the weights used in the different estimators. 
\end{remark}

% First a function $f_t$ is drawn from $D(\mathcal{F})$. The $t^\text{th}$ \textit{sequence} of tokens $\{\by_i\}_t$, is computed using a function $f_t$, that is $\by_{i, t} = (\bx_{i, t}, f_t(\bx_{i, t}))$. Here the $\{x_{i}\}_t$ are drawn from some data generation process. One of the tokens will be incomplete - $(\bx_{n}, 0)$ rather than $(\bx_n, f_t(\bx_n))$ - and the training accuracy of the model will be determined by how well $f_{SA}(\by_i)_{\bullet}$ predicts $f^*(\bx_i)$.


% each token  encodes a feature vector $\bx\in \mathbb{R}^d$ and a function value $f(\bx)$ concatenated together as $\mathbf{z}_i = (\bx_i, f(\bx_i))$. 

% The function $f$ is drawn from some distribution $D(\F)$ over a function class $\F$. We will refer to the element in the last coordinate of a token $\by$ as the token label, $\by_{\bullet}$. 



% TODO: deal with $\mathbf{W}_V$

% This is an established model to study in-context regression problems, studied also in {\color{red} TODO}. Many other analyses use this benign masking protocol \cite{huang2023context,cheng2023transformers}.



\begin{figure}
    \centering
    % \includegraphics[scale = 0.45, trim={3cm, 0, 3cm ,0}, clip]{Figures/tradeoff.pdf}
    \includegraphics[scale = 0.35]{Figures/tradeoff.pdf}
    \vspace{-4mm}
    \caption{From left to right, as we shrink the attention window (shaded in blue shading), the estimator has lower bias (shown in purple) but larger variance (shaded in tan).}
    \label{fig:tradeoff}
\end{figure}


% Note that while we do not explicitly indicate these dependencies in the notation, the map $\hat{f}_{SA}$ depends on every other token in the current sequence.



% softmax self-attention maps each token to three different vectors - the query-embedding, the key-embedding and the value embedding - via three linear mappings, $\mathbf{W}_Q, \mathbf{W}_K, \mathbf{W}_V$. {\color{red}We can think of these as establishing an associative container. ?} 
% Softmax attention maps a token $\bx$ by matching its query embedding with the key embeddings of other tokens, and returns a ``soft" value embedding of the resulting matches. Formally, softmax attention computes the matching between tokens $\bx_i$ and $\bx_j$ as $(\mathbf{W}_Q \bx_i)^\top (\mathbf{W}_K \bx_j)$, and uses this association to determine which of the value embeddings are important, as $\hat{f}_{SA}(\bx_i) \propto \sum_j \mathbf{W}_V\bx_je^{(\mathbf{W}_Q\bx_i)^\top (\mathbf{W}_K\bx_j)}.$ Finally, softmax attention normalizes the output by the sum of the association weights to yield 
% \begin{equation}\label{eq:attention}
% \hat{f}_{SA}(\bx_i) = \frac{\sum_j \mathbf{W}_V\bx_je^{(\mathbf{W}_Q\bx_i)^\top (\mathbf{W}_K\bx_j)}}{\sum_j e^{(\mathbf{W}_Q \bx_i)^\top (\mathbf{W}_K \bx_j)}}.
% \end{equation}Note that in this way, an attention layer maps every token $\bx_i$ to a token $\hat{f}_{SA}(\bx_i)$. 
% Note that while we do not explicitly indicate these dependencies in the notation, the map $\hat{f}_{SA}$ depends on every other token in the current sequence.


% \para{TODO: Linear self-attention and ICL as gradient descent.}
% A large number of recent works have studied ... 
% the special case of our  setting in which the functions $f$ are linear, that is, $f(\xi) = \mathbf{w}^\top \xi$ for some $\mathbf{w}\in \mathbb{R}^d$. 
%  These works analyze a simplified 


% This line of work has demonstrated both theoretically and empirically that one forward pass of in-context learning with  linear self-attention  can behave like running gradient descent using the context samples.  For example,

% However, this observation is specific to both linear self-attention and linear regression: once the labelling functions become nonlinear and/or the softmax activation is added, one forward pass of in-context learning is no longer equivalent to running gradient descent. We can see that in the linear regression case from above, inserting the softmax means the prediction is very different from the prediction of the gradient-descent-using linear attention:




% Thus,  a more general interpretation of the behavior of one-layer self-attention is necessary.



\begin{comment}
{\color{gray}


\para{Nearest Neighbours and Softmax:} There has been some work studying in-context learning with this model. For instance, it has been observed that such a model is able to learn \textit{to do linear regression} (as opposed to learning a single linear model). We show that what attention layers actually do is more general than this. We interpret the function $f_{SA}$ computed by the attention layer as behaving as a \textit{nearest neighbours predictor} that adapts to both the Lipschitzness of the functions it sees in training and the noise level. 

% {\color{red}We remark that this connection has been explored before, specifically in \cite{ahn2023transformers}, \cite{cheng2023transformers},} but not to the end of determining how this aids in-context learning.

Recall that the softmax attention prediction $f_{SA}(\bx_{n+1})$ (equation \ref{eq:attention}) is a weighted average  of the context labels, with weights determined by the exponentiated inner products $x_i^\top \mathbf{W}_K^\top \mathbf{W}_Q x_{n+1}$. The exponentiation has the effect of accentuating the weights of labels corresponding to relatively large $x_i^\top \mathbf{W}_K^\top \mathbf{W}_Q x_{n+1}$,  As  $\Vert \mathbf{W}_K^\top \mathbf{W}_Q\Vert$ increases, the softmax behaves more like a max, concentrating more weight on fewer, ``nearer" labels. 

As demonstrated in Figure \ref{fig:temperature}, the softmax allows us to select a scale for the neighborhood within which to average labels. For noisy labels generated by functions that change only slowly these neighborhoods should be large to average out the noise while still making an unbiased prediction. On the other hand, if the functions change rapidly, only labels of points close to the query contain information about the query label, so the softmax should average the labels of points in a relatively smaller neighborhood around the query.


}
\end{comment}



==> NearestNeighbours/Results.tex <==
\begin{section}{Results}
Our interpretation begins by rewriting Equation \ref{eq:attention} as 


\begin{equation}\label{eq:nearest_neighbour}
f_{SA}(\by_i)_{\cdot} = \frac{\sum_j f^*(\bx_j)e^{-w_{KQ}\Vert \bx_i-\bx_j\Vert^2}}{\sum_j e^{-w_{KQ}\Vert \bx_i-\bx_j\Vert^2}}
\end{equation}
We see that the output $f_{SA}(\by_i)_\cdot$ is determined by averaging the nearby known values of $f^*$. The scale of the averaging is determined by the parameter $w_{KQ}$. Here the model is faced with the following trade-off:
\begin{itemize}
\item Choosing a large constant $w_{KQ}$ will result in paying most attention to just a few nearby points. With little prior on the kinds of functions $f^*$ that the model is training on, these are the most important predicting the function value at $x_n$ - we will formalize this in the setting that the functions $f^*$ are Lipschitz.
\item Choosing a small $w_{KQ}$ will result in aggregating points from a larger neighborhood. When the target functions do not change rapidly, this is beneficial to reduce the variance in the estimator due to label noise.
\end{itemize}
We show that the attention layer adapts to the Lipschitzness of the functions $f_t$ seen in training. 
\begin{definition}[Lipschitzness of Function Class]
The Lipschitzness of a function class $\mathcal{F}$ and domain $\mathcal{X}$ is defined as the largest Lipschitz constant of all functions in $\mathcal{F}$ over the domain $\mathcal{X}$, that is:
    % Each $f_t\in \mathcal{F}$ is $L-$Lipschitz, that is 
   \begin{align} L(\mathcal{F}, \mathcal{X}) := \inf_{L \in \mathbb{R}} \{&L: f(x)-f(x')\le L\Vert x-x'\Vert \quad \forall (x,x') \in \mathcal{X}^2, f\in \mathcal{F}\}.\nonumber
    \end{align}
\end{definition}




% We also make the following assumption related to the spherical symmetry of the function class.
% \begin{assumption}
%     Each of the $f_t$ are such that $\mu(y) := \frac{\E_{x} f_t(x)e^{-\Vert x-y\Vert}}{\E_{x} e^{-\Vert x-y\Vert}}$ satisfies .
% \end{assumption}
We also make the following assumptions related to the rotational invariance of the function class.
% \begin{definition}\label{assump:rotation}
%     For any $x,x'\in \mathbb{S}^{d-1}$ and any rotation matrix ${R}\in \mathcal{O}^{d\times d}$, the following holds:
%     \begin{align*}
%         \mathbb{E}_{f \sim D(\mathcal{F})}[f_t(x)f_t(x')] =  \mathbb{E}_{f \sim D(\mathcal{F})}[f_t({R}x)f_t({R}x')].
%     \end{align*}
% \end{definition}

% \begin{definition}\label{assump:corr}
% For any $c > 0$ and $n\in \mathbb{Z}_+$, define $\mu_{c,n}(f_t, x) \coloneqq \mathbb{E}_{\{x_i\}_{i=1}^n\stackrel{\text{iid}}{\sim} \text{Unif}(\mathbb{S}^{d-1})}\left[\frac{f_t(x_1)\exp({c x_1^\top x})}{\sum_{i=1}^n \exp({c x_i^\top x}) }\right]$.
% For any $x,x'\in \mathbb{S}^{d-1}$ such that $x \neq x'$, 
% \begin{align*}
%     \mathbb{E}_{f \sim D(\mathcal{F})}[\mu_{c,n}(f_t,x)f_t(x)] >  \mathbb{E}_{f \sim D(\mathcal{F})}[\mu_{c,n}(f_t,x)f_t(x')].
% \end{align*}
% \end{definition}


% \begin{definition}[Rotational Invariance]\label{assump:rotation}
% For any function class $\mathcal{F}: \mathcal{X}\rightarrow \mathbb{R}$, the distribution $D(\mathcal{F})$ over $\mathcal{F}$ is  said to be {\em $B$-rotationally-invariant} if 
%     for any $x,x'\in \mathbb{S}^{d-1}$ and any rotation matrix ${R}\in \mathbb{O}^{k\times k}$, the following holds:
%     \begin{align*}
%         \mathbb{E}_{f \sim D(\mathcal{F})}[f(x)f(x')] =  \mathbb{E}_{f \sim D(\mathcal{F})}[f(B{R}B^\top x)f(B{R}B^\top x')].
%     \end{align*}
% \end{definition}
% definition \ref{assump:rotation} entails that for any fixed pair $(x,x')$, the correlation between $f(x)$ and $f(x')$  (with randomness due to choice of $f_t$) is invariant to identical rotations of $x$ and $x'$, in other words, $D(\mathcal{F})$ is in a sense spherically symmetric about the origin.
% % definition \ref{assump:rotation} entails that the correlation between $f_t(x)$ and $f_t(x')$  (with randomness due to choice of $f_t$) is invariant to identical rotations of $x$ and $x'$, in other words, $\mathcal{T}$ is spherically symmetric about the origin.

% \begin{definition}[$B$-regularity]\label{assump:corr}
% For any $c > 0$ and $n,d \in \mathbb{Z}_+^2$, define $$\mu_{c,n, d}(f, x) \coloneqq \mathbb{E}_{\{x_i\}_{i=1}^n\stackrel{\text{iid}}{\sim} \mathcal{U}^d}\left[\frac{f(x_1)\exp({c x_1^\top x})}{\sum_{i=1}^n \exp({c x_i^\top x}) }\right].$$
% For any function class $\mathcal{F}: \mathcal{X}\rightarrow \mathbb{R}$ that is rank-$k$ with support $B\in \mathbb{O}^{d \times k}$, the distribution $D(\mathcal{F})$ over $\mathcal{F}$ is  said to be {\em $B$-regular} if and $x,x'\in \mathcal{X}^2$ such that $x \neq x'$ satisfies
% \begin{align*}
%      \mathbb{E}_{f \sim D(\mathcal{F})}[\mu_{c,n}(f,x)f(x')] < \mathbb{E}_{f \sim D(\mathcal{F})}[\mu_{c,n}(f,x)f(x)].
% \end{align*}
% \end{definition}
% definition \ref{assump:corr} states that $\mu_{c,n}(f_t,x)$ is more correlated with $f_t(x)$ than $f_t(x')$ for any $x'\neq x$, where the randomness is due to the choice of $f_t$. Note that $\mu_{c,n}(f_t,x)$ is a weighted average of  $f_t(x_1)$ across $x_1$ on the unit hypersphere, where the weights scale exponentially with $x_1^T x$, so  $\mu_{c,n}(f_t,x)$ can be thought of as a prediction of $f_t(x)$, so it is natural to assume that $\mu_{c,n }(f_t,x)$ is more correlated with $f_t(x)$ than $f_t(x')$ for any other $x'$.





Finally, we assume the following about the distribution of $\by$.
\begin{assumption}
    Let $\uU$ denote the uniform distribution over the d dimensional hypersphere $\mathbb{S}^{d-1}$. Then $\by\sim\uU$.
\end{assumption}










We have seen in Section \ref{sec:formulation} that the prediction of the label of $\by$ output by one layer of softmax self-attention given context $X$ can be viewed as the prediction of a nearest neighbors regression. However, softmax attention still has $\Theta(d^2)$ degrees of freedom in the key and query matrices $W_K$ and $W_Q$ through which it can drastically manipulate the nature of the nearest neighbors regression. As we discussed earlier, softmax self-attention places more weight on fewer in-context samples as the eigenvalues of $W_K^\top W_Q$, meaning it effectively uses a smaller neighborhood size for nearest neighbors regression.
Our main result is the following:
\begin{quote}
    {\em During pre-training, one layer self-attention learns the appropriate neighborhood location and size for in-context learning via nearest neighbors regression, which is determined by the direction-wise Lipschitzness of the target function class.}
\end{quote}
% In  other words, during pre-training, 
We demonstrate this result theoretically in two ways: (i) we prove that if the target function class belongs to a  general family of nonlinear functions, the optimal $W_Q^\top W_K$ during pre-training  scales with the Lipschitzness of the function class, and (ii) when the target  function class includes only linear functions that share a common low-dimensional structure such that it has direction-wise Lipschitzness  of zero in all but $k< d$ directions, we show that the optimal $W_K^\top W_Q$ during pre-training is zero in all the zero-Lipschitzness directions.






% \subsection{Optimal $W_K^\top W_Q$ is scalar times identity}

% [scaled identity result here. or don't have a separate result for this]


% \subsection{Positive Results}
% We explore some of the consequences of this interpretation.

% \begin{comment}
    

\subsection{Softmax attention learns Lipschitz constant}






To highlight the important of the softmax in Theorem \ref{thm:}, we next show that linear attention cannot be guaranteed to learn anything meaningful when trained on function classes belonging to the family considered in Theorem \ref{thm:}.
\begin{theorem}\label{thm:negative-lin}
    Consider any function class consisting of odd functions, that is, any $\mathcal{F}$ such that for all $f \in \mathcal{F}$, $ f(x) = f(-x)$ for all $ x,x' \in \mathcal{X}$. Then $(W_K, W_Q)$ is a minimizer of $\mathcal{L}_{LA}(W_K, W_Q)$ if and only if $W_K^\top W_Q = 0$. Further, $\min_{W_K, W_Q} \mathcal{L}_{LA}(W_K, W_Q) = \frac{2+ \sigma^2}{n}$. 
\end{theorem}
Theorem \ref{thm:negative-lin} shows that linear attention cannot learn anything meaningful when the tasks are odd functions. Examples of such function classes are


% \end{comment}


% \subsubsection{Empirical generalization}


\end{section}

==> tikz_styles.tex <==
\tikzstyle{phantom vertex} = [ ellipse, 
                               anchor = center, 
                               minimum height = 1*\unit, 
                               minimum width  = 1*\unit,
                               inner sep=0pt,
                               anchor=center]
\tikzstyle{red vertex}   = [black, fill = red!20,   phantom vertex, draw]
\tikzstyle{black vertex} = [black, fill = black!20, phantom vertex, draw]
\tikzstyle{blue vertex}  = [black, fill = blue!20,  phantom vertex, draw]
\tikzstyle{green vertex} = [black, fill = green!20,  phantom vertex, draw]
\tikzstyle{vertex}       = [draw, phantom vertex]

\tikzstyle{point} = [ellipse, inner sep=0pt, draw, fill=white, anchor = center,
                     minimum height = 0.05*\unit, minimum width  = 0.05*\unit]
                     
